Higher local systems and the categorified monodromy equivalence

We study local systems of $(\infty,n)$-categories on spaces. We prove that categorical local systems are captured by (higher) monodromy data: in particular, if $X$ is $(n+1)$-connected, then local systems of $(\infty,n)$-categories over $X$ can be described as $\mathbb{E}_{n+1}$-modules over the iterated loop space $\Omega_{n+1}X$. This generalizes the classical monodromy equivalence presenting ordinary local systems as modules over the based loop spaces. Along the way we revisit from the perspective of $\infty$-categories Teleman's influential theory of topological group actions on categories, and we extend it to topological actions on $(\infty,n)$-categories. Finally, we show that the group of invertible objects in the category of local systems of $(\infty,n)$-categories over an $n$-connected space $X$ is isomorphic to the group of characters of $\pi_n(X)$. This should be thought of as a topological analogue of the higher Brauer group of the space $X$. We conclude the paper with applications of the theory of categorical local systems to the fiberwise Fukaya category of symplectic fibrations.

==> Bibliography.tex <==


@misc{preygel2011thomsebastianidualitymatrix,
      title={Thom-Sebastiani and Duality for Matrix Factorizations}, 
      author={Anatoly Preygel},
      year={2011},
      eprint={1101.5834},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/1101.5834}, 
}

@article {neeman_grothendieck_duality,
    AUTHOR = {Neeman, Amnon},
     TITLE = {The {G}rothendieck duality theorem via {B}ousfield's
              techniques and {B}rown representability},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {9},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {205--236},
      ISSN = {0894-0347,1088-6834},
   MRCLASS = {18E30 (14F05)},
  MRNUMBER = {1308405},
MRREVIEWER = {Luca\ Barbieri Viale},
       DOI = {10.1090/S0894-0347-96-00174-9},
       URL = {https://doi.org/10.1090/S0894-0347-96-00174-9},
}

@article {serre2,
    AUTHOR = {Serre, Jean-Pierre},
     TITLE = {Un th\'eor\`eme de dualit\'e},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {29},
      YEAR = {1955},
     PAGES = {9--26},
      ISSN = {0010-2571,1420-8946},
   MRCLASS = {56.0X},
  MRNUMBER = {67489},
MRREVIEWER = {S.\ Chern},
       DOI = {10.1007/BF02564268},
       URL = {https://doi.org/10.1007/BF02564268},
}


@article {braden2016conical,
    AUTHOR = {Braden, Tom and Licata, Anthony and Proudfoot, Nicholas and
              Webster, Ben},
     TITLE = {Quantizations of conical symplectic resolutions {II}: category
              {$\mathcal{O}$} and symplectic duality},
      NOTE = {with an appendix by I. Losev},
   JOURNAL = {Ast\'erisque},
  FJOURNAL = {Ast\'erisque},
    NUMBER = {384},
      YEAR = {2016},
     PAGES = {75--179},
      ISSN = {0303-1179,2492-5926},
      ISBN = {978-2-85629-845-9},
   MRCLASS = {53D50 (14F05 14J81 16S38 17B10)},
  MRNUMBER = {3594665},
}






@article {MR2430869,
    AUTHOR = {Lu, Di Ming and Palmieri, John H. and Wu, Quan Shui and Zhang,
              James J.},
     TITLE = {Koszul equivalences in {$A_\infty$}-algebras},
   JOURNAL = {New York J. Math.},
  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {14},
      YEAR = {2008},
     PAGES = {325--378},
      ISSN = {1076-9803},
   MRCLASS = {16E45 (16E35 16S37)},
  MRNUMBER = {2430869},
MRREVIEWER = {Mikael\ Vejdemo Johansson},
       URL = {http://nyjm.albany.edu:8000/j/2008/14_325.html},
}

@misc{Pascaleff_Pavia_Sibilla_Koszul,
AUTHOR={Pascaleff, James and Pavia, Emanuele and Sibilla, Nicolò},
TITLE={Higher Koszul duality via $n$-affineness},
YEAR={2025},
}

@misc{Pascaleff_Pavia_Sibilla_Local_Systems,
AUTHOR={Pascaleff, James and Pavia, Emanuele and Sibilla, Nicolò},
TITLE={Higher local systems and categorified monodromy equivalence},
YEAR={2025},
}




@book {sabbah,
    AUTHOR = {Sabbah, Claude},
     TITLE = {Isomonodromic deformations and {F}robenius manifolds},
    SERIES = {Universitext},
   EDITION = {French},
      NOTE = {An introduction},
 PUBLISHER = {Springer-Verlag London, Ltd., London; EDP Sciences, Les Ulis},
      YEAR = {2007},
     PAGES = {xiv+279},
      ISBN = {978-1-84800-053-7; 978-2-7598-0047-6},
   MRCLASS = {32G34 (32S30 32S40 33E50 34M45 53D45)},
  MRNUMBER = {2368364},
}


	@misc{pavia1,
	doi = {10.48550/ARXIV.2207.11994},
	url = {https://arxiv.org/abs/2207.11994},
	author = {Pavia, Emanuele},
	keywords = {Category Theory (math.CT), Algebraic Geometry (math.AG), K-Theory and Homology (math.KT), FOS: Mathematics, FOS: Mathematics},
	title = {A $t$-structure on the $\infty$-category of mixed graded modules},
	publisher = {arXiv},
	year = {2022},
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{pavia2,
title = {Mixed graded structure on Chevalley-Eilenberg functors},
journal = {Advances in Mathematics},
volume = {448},
pages = {109721},
year = {2024},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2024.109721},
url = {https://www.sciencedirect.com/science/article/pii/S0001870824002366},
author = {Emanuele Pavia},
}


@article {compositionproduct,
	AUTHOR = {Haugseng, Rune},
	TITLE = {{$\infty$}-operads via symmetric sequences},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {301},
	YEAR = {2022},
	NUMBER = {1},
	PAGES = {115--171},
	ISSN = {0025-5874},
	MRCLASS = {18N70},
	MRNUMBER = {4405646},
	DOI = {10.1007/s00209-021-02881-w},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1007/s00209-021-02881-w},
}


@article {geometryoffiltrations,
	AUTHOR = {Moulinos, Tasos},
	TITLE = {The geometry of filtrations},
	JOURNAL = {Bull. Lond. Math. Soc.},
	FJOURNAL = {Bulletin of the London Mathematical Society},
	VOLUME = {53},
	YEAR = {2021},
	NUMBER = {5},
	PAGES = {1486--1499},
	ISSN = {0024-6093},
	MRCLASS = {14F08 (14A20 55P42)},
	MRNUMBER = {4335221},
	DOI = {10.1112/blms.12512},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1112/blms.12512},
}


@article {fubini,
	AUTHOR = {Chach\'{o}lski, Wojciech and Scherer, J\'{e}r\^{o}me},
	TITLE = {Homotopy theory of diagrams},
	JOURNAL = {Mem. Amer. Math. Soc.},
	FJOURNAL = {Memoirs of the American Mathematical Society},
	VOLUME = {155},
	YEAR = {2002},
	NUMBER = {736},
	PAGES = {x+90},
	ISSN = {0065-9266},
	MRCLASS = {55P65 (18G55 55U30)},
	MRNUMBER = {1879153},
	MRREVIEWER = {Timothy Porter},
	DOI = {10.1090/memo/0736},
	URL = {https://doi.org/10.1090/memo/0736},
}


@book {tannakaduality,
	AUTHOR = {Schauenburg, Peter},
	TITLE = {Tannaka duality for arbitrary {H}opf algebras},
	SERIES = {Algebra Berichte [Algebra Reports]},
	VOLUME = {66},
	PUBLISHER = {Verlag Reinhard Fischer, Munich},
	YEAR = {1992},
	PAGES = {ii+57},
	ISBN = {3-88927-100-6},
	MRCLASS = {18D10 (16W30 18F99)},
	MRNUMBER = {1623637},
}


@misc{bialgebrasmonoidalstructure,
	doi = {10.48550/ARXIV.1810.00734},
	url = {https://arxiv.org/abs/1810.00734},
	author = {Beardsley, Jonathan},
	keywords = {Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics, 55N22, 55P43, 16T10, 18N70, 18F20},
	title = {On Bialgebras, Comodules, Descent Data and Thom Spectra in $\infty$-categories},
	publisher = {arXiv},
	year = {2018},	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{yonedaisnatural1,
	doi = {10.48550/ARXIV.2011.11042},
	
	url = {https://arxiv.org/abs/2011.11042},
	
	author = {Haugseng, Rune and Hebestreit, Fabian and Linskens, Sil and Nuiten, Joost},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics, 18N60, 18N70},
	
	title = {Two-variable fibrations, factorisation systems and $\infty$-categories of spans},
	
	publisher = {arXiv},
	
	year = {2020},
	
	copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}


@misc{yonedaisnatural2,
	doi = {10.48550/ARXIV.2209.12575},
	
	url = {https://arxiv.org/abs/2209.12575},
	
	author = {Ramzi, Maxime},
	
	keywords = {Category Theory (math.CT), FOS: Mathematics, FOS: Mathematics},
	
	title = {The Yoneda embedding is natural},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{yonedaisnatural3,
	doi = {10.48550/ARXIV.2301.00601},
	
	url = {https://arxiv.org/abs/2301.00601},
	
	author = {Moshe, Shay Ben},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics},
	
	title = {Naturality of the $\infty$-Categorical Enriched Yoneda Embedding},
	
	publisher = {arXiv},
	
	year = {2023},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}




@misc{koszulduality,
  doi = {10.48550/ARXIV.1909.11724},
    url = {https://arxiv.org/abs/1909.11724},
    author = {Beardsley, Jonathan and Péroux, Maximilien},
    keywords = {Algebraic Topology (math.AT), Category Theory (math.CT), FOS: Mathematics, FOS: Mathematics, 55U30, 16T15},
    title = {Koszul Duality in Higher Topoi},
    publisher = {arXiv},
    year = {2019},
    copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings {teleman,
    AUTHOR = {Teleman, Constantin},
     TITLE = {Gauge theory and mirror symmetry},
 BOOKTITLE = {Proceedings of the {I}nternational {C}ongress of
              {M}athematicians---{S}eoul 2014. {V}ol. {II}},
     PAGES = {1309--1332},
 PUBLISHER = {Kyung Moon Sa, Seoul},
      YEAR = {2014},
   MRCLASS = {57R56 (18D05 55N91)},
  MRNUMBER = {3728663},
MRREVIEWER = {Ramses Fernandez-Valencia},
}


@book {MR1896125,
    AUTHOR = {Polcino Milies, C\'esar and Sehgal, Sudarshan K.},
     TITLE = {An introduction to group rings},
    SERIES = {Algebra and Applications},
    VOLUME = {1},
 PUBLISHER = {Kluwer Academic Publishers, Dordrecht},
      YEAR = {2002},
     PAGES = {xii+371},
      ISBN = {1-4020-0238-6},
   MRCLASS = {16S34 (16-01 16U60)},
  MRNUMBER = {1896125},
MRREVIEWER = {Edgar\ G.\ Goodaire},
       DOI = {10.1007/978-94-010-0405-3},
       URL = {https://doi.org/10.1007/978-94-010-0405-3},
}


@article {rezk1,
    AUTHOR = {Bergner, Julia E. and Rezk, Charles},
     TITLE = {Comparison of models for {$(\infty,n)$}-categories, {I}},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {17},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {2163--2202},
      ISSN = {1465-3060},
   MRCLASS = {18D05 (18G55)},
  MRNUMBER = {3109865},
MRREVIEWER = {Javier J. Guti\'{e}rrez},
       DOI = {10.2140/gt.2013.17.2163},
       URL = {https://doi.org/10.2140/gt.2013.17.2163},
}
@article {rezk2,
    AUTHOR = {Bergner, Julia E. and Rezk, Charles},
     TITLE = {Comparison of models for {$(\infty, n)$}-categories, {II}},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {13},
      YEAR = {2020},
    NUMBER = {4},
     PAGES = {1554--1581},
      ISSN = {1753-8416},
   MRCLASS = {18N65 (18N40 55U35 55U40)},
  MRNUMBER = {4186138},
       DOI = {10.1112/topo.12167},
       URL = {https://doi.org/10.1112/topo.12167},
}


@article {dualizingcartcocart,
	AUTHOR = {Barwick, Clark and Glasman, Saul and Nardin, Denis},
	TITLE = {Dualizing cartesian and cocartesian fibrations},
	JOURNAL = {Theory Appl. Categ.},
	FJOURNAL = {Theory and Applications of Categories},
	VOLUME = {33},
	YEAR = {2018},
	PAGES = {Paper No. 4, 67--94},
	MRCLASS = {18D15},
	MRNUMBER = {3746613},
	MRREVIEWER = {Josep Elgueta},
}


@article {colie,
	AUTHOR = {Ho, Quoc P.},
	TITLE = {Homological stability and densities of generalized
		configuration spaces},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {25},
	YEAR = {2021},
	NUMBER = {2},
	PAGES = {813--912},
	ISSN = {1465-3060},
	MRCLASS = {14F35 (14G05 17B62 55P62 55R80)},
	MRNUMBER = {4251437},
	DOI = {10.2140/gt.2021.25.813},
	URL = {https://doi-org.pros1.lib.unimi.it/10.2140/gt.2021.25.813},
}


@incollection {lagcorr,
	AUTHOR = {Calaque, Damien},
	TITLE = {Lagrangian structures on mapping stacks and semi-classical
		{TFT}s},
	BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
	SERIES = {Contemp. Math.},
	VOLUME = {643},
	PAGES = {1--23},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {2015},
	MRCLASS = {53D12 (14A20 14F05 81T45)},
	MRNUMBER = {3381468},
	MRREVIEWER = {Brent Pym},
	DOI = {10.1090/conm/643/12894},
	URL = {https://doi.org/10.1090/conm/643/12894},
}


@article {BRST,
	AUTHOR = {Fuster, Andrea and Henneaux, Marc and Maas, Axel},
	TITLE = {B{RST}-antifield quantization: a short review},
	JOURNAL = {Int. J. Geom. Methods Mod. Phys.},
	FJOURNAL = {International Journal of Geometric Methods in Modern Physics},
	VOLUME = {2},
	YEAR = {2005},
	NUMBER = {5},
	PAGES = {939--963},
	ISSN = {0219-8878},
	MRCLASS = {81T70 (81-02 81T13)},
	MRNUMBER = {2177293},
	MRREVIEWER = {Beatrice Bucker},
	DOI = {10.1142/S0219887805000892},
	URL = {https://doi.org/10.1142/S0219887805000892},
}


@article {BRST2,
	AUTHOR = {Barnich, Glenn and Brandt, Friedemann and Henneaux, Marc},
	TITLE = {Local {BRST} cohomology in gauge theories},
	JOURNAL = {Phys. Rep.},
	FJOURNAL = {Physics Reports. A Review Section of Physics Letters},
	VOLUME = {338},
	YEAR = {2000},
	NUMBER = {5},
	PAGES = {439--569},
	ISSN = {0370-1573},
	MRCLASS = {81T70 (17B81 81-02)},
	MRNUMBER = {1792979},
	MRREVIEWER = {Bani Mitra S\"{o}dermark},
	DOI = {10.1016/S0370-1573(00)00049-1},
	URL = {https://doi.org/10.1016/S0370-1573(00)00049-1},
}


@article {cyclichomology,
	AUTHOR = {Kassel, Christian},
	TITLE = {Cyclic homology, comodules, and mixed complexes},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {107},
	YEAR = {1987},
	NUMBER = {1},
	PAGES = {195--216},
	ISSN = {0021-8693},
	MRCLASS = {18G35 (19D55 55U25)},
	MRNUMBER = {883882},
	MRREVIEWER = {Sue Geller},
	DOI = {10.1016/0021-8693(87)90086-X},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/0021-8693(87)90086-X},
}


@article {burghelea,
	AUTHOR = {Burghelea, Dan and Ogle, Crichton},
	TITLE = {The {K}\"{u}nneth formula in cyclic homology},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {193},
	YEAR = {1986},
	NUMBER = {4},
	PAGES = {527--536},
	ISSN = {0025-5874},
	MRCLASS = {18F25 (18G15 19D55)},
	MRNUMBER = {867346},
	MRREVIEWER = {Claude Schochet},
	DOI = {10.1007/BF01160473},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1007/BF01160473},
}


@article {coalgebrascomonad,
	AUTHOR = {Hess, Kathryn and Shipley, Brooke},
	TITLE = {The homotopy theory of coalgebras over a comonad},
	JOURNAL = {Proc. Lond. Math. Soc. (3)},
	FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
	VOLUME = {108},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {484--516},
	ISSN = {0024-6115},
	MRCLASS = {55U35 (16T15 18C15 18G55 55U15)},
	MRNUMBER = {3166360},
	MRREVIEWER = {Javier J. Guti\'{e}rrez},
	DOI = {10.1112/plms/pdt038},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/plms/pdt038},
}


@mastersthesis{ozbek,
	title={The Homotopy Theory of Commutative dg Algebras and Representability Theorems for Lie Algebra Cohomology},
	author={Aydin Ozbek},
	year={2016},
	school={University of Nevada, Reno},
%	address={XXX}
}


@article {brown,
	AUTHOR = {Brown, Kenneth S.},
	TITLE = {Abstract homotopy theory and generalized sheaf cohomology},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {186},
	YEAR = {1973},
	PAGES = {419--458},
	ISSN = {0002-9947},
	MRCLASS = {55B30 (18H99)},
	MRNUMBER = {341469},
	MRREVIEWER = {A. Dold},
	DOI = {10.2307/1996573},
	URL = {https://doi-org.pros.lib.unimi.it/10.2307/1996573},
}


@misc{hinichdayconvolution,
	doi = {10.48550/ARXIV.2101.09538},
	
	url = {https://arxiv.org/abs/2101.09538},
	
	author = {Hinich, Vladimir},
	
	keywords = {Category Theory (math.CT), Quantum Algebra (math.QA), FOS: Mathematics, FOS: Mathematics, 18D20, 18N60, 18N70},
	
	title = {Colimits in enriched $\infty$-categories and Day convolution},
	
	publisher = {arXiv},
	
	year = {2021},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}




@article {riehl2,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Infinity category theory from scratch},
	JOURNAL = {High. Struct.},
	FJOURNAL = {Higher Structures},
	VOLUME = {4},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {115--167},
	MRCLASS = {18N60 (18A30 18A40 55U35)},
	MRNUMBER = {4074275},
}

@article {homotopycoherentadj,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Homotopy coherent adjunctions and the formal theory of monads},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {286},
	YEAR = {2016},
	PAGES = {802--888},
	ISSN = {0001-8708},
	MRCLASS = {18G55 (18C15 55U10 55U35 55U40)},
	MRNUMBER = {3415698},
	MRREVIEWER = {R. H. Street},
	DOI = {10.1016/j.aim.2015.09.011},
	URL = {https://doi.org/10.1016/j.aim.2015.09.011},
}

@article {CS,
	AUTHOR = {Canonaco, Alberto and Stellari, Paolo},
	TITLE = {Uniqueness of dg enhancements for the derived category of a
		{G}rothendieck category},
	JOURNAL = {J. Eur. Math. Soc. (JEMS)},
	FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
	VOLUME = {20},
	YEAR = {2018},
	NUMBER = {11},
	PAGES = {2607--2641},
	ISSN = {1435-9855},
	MRCLASS = {14F05 (18E10 18E30)},
	MRNUMBER = {3861804},
	MRREVIEWER = {Jon Eivind Vatne},
	DOI = {10.4171/JEMS/820},
	URL = {https://doi.org/10.4171/JEMS/820},
}

@article {duggershipley,
	AUTHOR = {Dugger, Daniel and Shipley, Brooke},
	TITLE = {A curious example of triangulated-equivalent model categories
		which are not {Q}uillen equivalent},
	JOURNAL = {Algebr. Geom. Topol.},
	FJOURNAL = {Algebraic \& Geometric Topology},
	VOLUME = {9},
	YEAR = {2009},
	NUMBER = {1},
	PAGES = {135--166},
	ISSN = {1472-2747},
	MRCLASS = {18E30 (18F25 55U35)},
	MRNUMBER = {2482071},
	MRREVIEWER = {Mark Hovey},
	DOI = {10.2140/agt.2009.9.135},
	URL = {https://doi.org/10.2140/agt.2009.9.135},
}

@article {rizzardovdb,
	AUTHOR = {Rizzardo, Alice and Van den Bergh, Michel},
	TITLE = {A note on non-unique enhancements},
	JOURNAL = {Proc. Amer. Math. Soc.},
	FJOURNAL = {Proceedings of the American Mathematical Society},
	VOLUME = {147},
	YEAR = {2019},
	NUMBER = {2},
	PAGES = {451--453},
	ISSN = {0002-9939},
	MRCLASS = {18E30 (13D09 14A22)},
	MRNUMBER = {3894882},
	MRREVIEWER = {Mee Seong Im},
	DOI = {10.1090/proc/14065},
	URL = {https://doi.org/10.1090/proc/14065},
}

@article {schwedemodel2,
	AUTHOR = {Schwede, Stefan},
	TITLE = {The stable homotopy category has a unique model at the prime
		2},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {164},
	YEAR = {2001},
	NUMBER = {1},
	PAGES = {24--40},
	ISSN = {0001-8708},
	MRCLASS = {55P42 (18G55 55U35)},
	MRNUMBER = {1870511},
	MRREVIEWER = {A. D. Elmendorf},
	DOI = {10.1006/aima.2001.2009},
	URL = {https://doi.org/10.1006/aima.2001.2009},
}

@article {mazelgee,
	AUTHOR = {Mazel-Gee, Aaron},
	TITLE = {Quillen adjunctions induce adjunctions of quasicategories},
	JOURNAL = {New York J. Math.},
	FJOURNAL = {New York Journal of Mathematics},
	VOLUME = {22},
	YEAR = {2016},
	PAGES = {57--93},
	MRCLASS = {18A40},
	MRNUMBER = {3484677},
	MRREVIEWER = {Srikanth B. Iyengar},
	URL = {http://p8000-nyjm.albany.edu.pros1.lib.unimi.it/j/2016/22_57.html},
}

@book {elementsofinftycat,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Elements of {$\infty$}-category theory},
	SERIES = {Cambridge Studies in Advanced Mathematics},
	VOLUME = {194},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2022},
	PAGES = {xix+759},
	ISBN = {978-1-108-83798-9},
	MRCLASS = {18-02 (18Nxx)},
	MRNUMBER = {4354541},
	DOI = {10.1017/9781108936880},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1017/9781108936880},
}

@misc{rezkquasicat,
AUTHOR = {Rezk, Charles},
TITLE = {Introduction to quasicategories},
YEAR={2021},
URL={https://people.math.rochester.edu/faculty/doug/otherpapers/Rezk-quasicats-intro.pdf},
}

@incollection {gepner,
    AUTHOR = {Gepner, David},
     TITLE = {An introduction to higher categorical algebra},
 BOOKTITLE = {Handbook of homotopy theory},
    SERIES = {CRC Press/Chapman Hall Handb. Math. Ser.},
     PAGES = {487--548},
 PUBLISHER = {CRC Press, Boca Raton, FL},
      YEAR = {2020},
      ISBN = {978-0-815-36970-7},
   MRCLASS = {55U35 (16E45 18C10 18C35)},
  MRNUMBER = {4197993},
MRREVIEWER = {Thomas\ H\"uttemann},
}

@article {milnor,
    AUTHOR = {Milnor, John},
     TITLE = {The geometric realization of a semi-simplicial complex},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {65},
      YEAR = {1957},
     PAGES = {357--362},
      ISSN = {0003-486X},
   MRCLASS = {55.0X},
  MRNUMBER = {84138},
MRREVIEWER = {J.\ C.\ Moore},
       DOI = {10.2307/1969967},
       URL = {https://doi.org/10.2307/1969967},
}

@incollection {joyal,
	AUTHOR = {Joyal, A.},
	TITLE = {Quasi-categories and {K}an complexes},
	NOTE = {Special volume celebrating the 70th birthday of Professor Max
		Kelly},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {175},
	YEAR = {2002},
	NUMBER = {1-3},
	PAGES = {207--222},
	ISSN = {0022-4049},
	MRCLASS = {55U10 (18G55)},
	MRNUMBER = {1935979},
	MRREVIEWER = {Donald M. Davis},
	DOI = {10.1016/S0022-4049(02)00135-4},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/S0022-4049(02)00135-4},
}

@book {maysimplicial,
    AUTHOR = {May, J. Peter},
     TITLE = {Simplicial objects in algebraic topology},
    SERIES = {Van Nostrand Mathematical Studies},
    VOLUME = {No. 11},
 PUBLISHER = {D. Van Nostrand Co., Inc., Princeton, N.J.-Toronto,
              Ont.-London},
      YEAR = {1967},
     PAGES = {vi+161},
   MRCLASS = {55.40},
  MRNUMBER = {222892},
MRREVIEWER = {A.\ K.\ Bousfield},
}

@book {riehl3,
	AUTHOR = {Riehl, Emily},
	TITLE = {Categorical homotopy theory},
	SERIES = {New Mathematical Monographs},
	VOLUME = {24},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2014},
	PAGES = {xviii+352},
	ISBN = {978-1-107-04845-4},
	MRCLASS = {18G55 (18D20 55U35)},
	MRNUMBER = {3221774},
	MRREVIEWER = {David A. Blanc},
	DOI = {10.1017/CBO9781107261457},
	URL = {https://doi.org/10.1017/CBO9781107261457},
}


@article {GHN,
	AUTHOR = {Gepner, David and Haugseng, Rune and Nikolaus, Thomas},
	TITLE = {Lax colimits and free fibrations in {$\infty$}-categories},
	JOURNAL = {Doc. Math.},
	FJOURNAL = {Documenta Mathematica},
	VOLUME = {22},
	YEAR = {2017},
	PAGES = {1225--1266},
	ISSN = {1431-0635},
	MRCLASS = {18D30 (18A30)},
	MRNUMBER = {3690268},
	MRREVIEWER = {Josep Elgueta},
}


@misc{laxmonoidal,
	doi = {10.48550/ARXIV.2011.08808},
	
	url = {https://arxiv.org/abs/2011.08808},
	
	author = {Haugseng, Rune and Hebestreit, Fabian and Linskens, Sil and Nuiten, Joost},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics},
	
	title = {Lax monoidal adjunctions, two-variable fibrations and the calculus of mates},
	
	publisher = {arXiv},
	
	year = {2020},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@book {riehlverity,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Elements of {$\infty$}-category theory},
	SERIES = {Cambridge Studies in Advanced Mathematics},
	VOLUME = {194},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2022},
	PAGES = {xix+759},
	ISBN = {978-1-108-83798-9},
	MRCLASS = {18-02 (18Nxx)},
	MRNUMBER = {4354541},
	DOI = {10.1017/9781108936880},
	URL = {https://doi.org/10.1017/9781108936880},
}


@article {riehl,
	AUTHOR = {Ching, Michael and Riehl, Emily},
	TITLE = {Coalgebraic models for combinatorial model categories},
	JOURNAL = {Homology Homotopy Appl.},
	FJOURNAL = {Homology, Homotopy and Applications},
	VOLUME = {16},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {171--184},
	ISSN = {1532-0073},
	MRCLASS = {18C35},
	MRNUMBER = {3257572},
	MRREVIEWER = {George Ciprian Modoi},
	DOI = {10.4310/HHA.2014.v16.n2.a9},
	URL = {https://doi.org/10.4310/HHA.2014.v16.n2.a9},
}


@misc{derivedfoliations2,
	title={Algebraic foliations and derived geometry II: the Grothendieck-Riemann-Roch theorem},
	author={Bertrand Toën and Gabriele Vezzosi},
	year={2020},
	eprint={2007.09251},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@misc{toen2020algebraic,
	title={Algebraic foliations and derived geometry I: the Riemann-Hilbert correspondence}, 
	author={Bertrand Toën and Gabriele Vezzosi},
	year={2020},
	eprint={2001.05450},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@article {krizmay,
	AUTHOR = {K\v{r}\'{\i}\v{z}, Igor and May, J. P.},
	TITLE = {Operads, algebras, modules and motives},
	JOURNAL = {Ast\'{e}risque},
	FJOURNAL = {Ast\'{e}risque},
	NUMBER = {233},
	YEAR = {1995},
	PAGES = {iv+145pp},
	ISSN = {0303-1179},
	MRCLASS = {18G99 (14F99 19E99 55U99)},
	MRNUMBER = {1361938},
	MRREVIEWER = {J. P. C. Greenlees},
}


@article {dwyerkan,
	AUTHOR = {Dwyer, W. G. and Kan, D. M.},
	TITLE = {Calculating simplicial localizations},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {18},
	YEAR = {1980},
	NUMBER = {1},
	PAGES = {17--35},
	ISSN = {0022-4049},
	MRCLASS = {55U35 (18D20)},
	MRNUMBER = {578563},
	MRREVIEWER = {Timothy Porter},
	DOI = {10.1016/0022-4049(80)90113-9},
	URL = {https://doi-org.pros.lib.unimi.it/10.1016/0022-4049(80)90113-9},
}


@article {ching,
	AUTHOR = {Ching, Michael},
	TITLE = {Bar-cobar duality for operads in stable homotopy theory},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {5},
	YEAR = {2012},
	NUMBER = {1},
	PAGES = {39--80},
	ISSN = {1753-8416},
	MRCLASS = {55P48 (18D50 55P42)},
	MRNUMBER = {2897049},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.1112/jtopol/jtr027},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/jtopol/jtr027},
}


@article {baranovsky,
	AUTHOR = {Baranovsky, Vladimir},
	TITLE = {A universal enveloping for {$L_\infty$}-algebras},
	JOURNAL = {Math. Res. Lett.},
	FJOURNAL = {Mathematical Research Letters},
	VOLUME = {15},
	YEAR = {2008},
	NUMBER = {6},
	PAGES = {1073--1089},
	ISSN = {1073-2780},
	MRCLASS = {18G55 (17B55)},
	MRNUMBER = {2470385},
	MRREVIEWER = {Wendy Lowen},
	DOI = {10.4310/MRL.2008.v15.n6.a1},
	URL = {https://doi-org.pros.lib.unimi.it/10.4310/MRL.2008.v15.n6.a1},
}


@article {modelstructureforgoldmanmillson,
	AUTHOR = {Robert-Nicoud, Daniel},
	TITLE = {A model structure for the {G}oldman-{M}illson theorem},
	JOURNAL = {Grad. J. Math.},
	FJOURNAL = {The Graduate Journal of Mathematics},
	VOLUME = {3},
	YEAR = {2018},
	NUMBER = {1},
	PAGES = {15--30},
	MRCLASS = {18G55 (17B55)},
	MRNUMBER = {3876592},
	MRREVIEWER = {Zuhier Khaled Altawallbeh},
}


@article {stronglyhomotopyliealgebras,
	AUTHOR = {Lada, Tom and Markl, Martin},
	TITLE = {Strongly homotopy {L}ie algebras},
	JOURNAL = {Comm. Algebra},
	FJOURNAL = {Communications in Algebra},
	VOLUME = {23},
	YEAR = {1995},
	NUMBER = {6},
	PAGES = {2147--2161},
	ISSN = {0092-7872},
	MRCLASS = {16S30 (17B35 18G99)},
	MRNUMBER = {1327129},
	MRREVIEWER = {Stanis\l aw Betley},
	DOI = {10.1080/00927879508825335},
	URL = {https://doi-org.pros.lib.unimi.it/10.1080/00927879508825335},
}


@article {linearbatalin,
	AUTHOR = {Gwilliam, Owen and Haugseng, Rune},
	TITLE = {Linear {B}atalin-{V}ilkovisky quantization as a functor of
		{$\infty$}-categories},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {24},
	YEAR = {2018},
	NUMBER = {2},
	PAGES = {1247--1313},
	ISSN = {1022-1824},
	MRCLASS = {18G55 (14D23 17B37 18D50 53D55 58J52 81Q99 81T70)},
	MRNUMBER = {3782422},
	MRREVIEWER = {Olga Kravchenko},
	DOI = {10.1007/s00029-018-0396-0},
	URL = {https://doi-org.pros.lib.unimi.it/10.1007/s00029-018-0396-0},
}


@article {chiralkoszul,
	AUTHOR = {Francis, John and Gaitsgory, Dennis},
	TITLE = {Chiral {K}oszul duality},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {18},
	YEAR = {2012},
	NUMBER = {1},
	PAGES = {27--87},
	ISSN = {1022-1824},
	MRCLASS = {14F10 (14F05 14H81 17B55 18D10 18D50)},
	MRNUMBER = {2891861},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.1007/s00029-011-0065-z},
	URL = {https://doi.org/10.1007/s00029-011-0065-z},
}


@article {rationalhomotopytheory,
	AUTHOR = {Quillen, Daniel},
	TITLE = {Rational homotopy theory},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {90},
	YEAR = {1969},
	PAGES = {205--295},
	ISSN = {0003-486X},
	MRCLASS = {55.40},
	MRNUMBER = {258031},
	MRREVIEWER = {J. F. Adams},
	DOI = {10.2307/1970725},
	URL = {https://doi-org.pros.lib.unimi.it/10.2307/1970725},
}


@article {priddykoszul,
    AUTHOR = {Priddy, Stewart B.},
     TITLE = {Koszul resolutions},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {152},
      YEAR = {1970},
     PAGES = {39--60},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {18.20},
  MRNUMBER = {265437},
MRREVIEWER = {A.\ K.\ Bousfield},
       DOI = {10.2307/1995637},
       URL = {https://doi.org/10.2307/1995637},
}


@article {enhancingfiltered,
	AUTHOR = {Gwilliam, Owen and Pavlov, Dmitri},
	TITLE = {Enhancing the filtered derived category},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {222},
	YEAR = {2018},
	NUMBER = {11},
	PAGES = {3621--3674},
	ISSN = {0022-4049},
	MRCLASS = {18E30 (18E10)},
	MRNUMBER = {3806745},
	MRREVIEWER = {Wolfgang Rump},
	DOI = {10.1016/j.jpaa.2018.01.004},
	URL = {https://doi-org.pros.lib.unimi.it:2050/10.1016/j.jpaa.2018.01.004},
}

@book {hatcher,
    AUTHOR = {Hatcher, Allen},
     TITLE = {Algebraic topology},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2002},
     PAGES = {xii+544},
      ISBN = {0-521-79540-0},
   MRCLASS = {55-01 (55-00)},
  MRNUMBER = {1867354},
MRREVIEWER = {Donald\ W.\ Kahn},
}

@book {coend,
	AUTHOR = {Loregian, Fosco},
	TITLE = {({C}o)end calculus},
	SERIES = {London Mathematical Society Lecture Note Series},
	VOLUME = {468},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2021},
	PAGES = {xxi+308},
	ISBN = {978-1-108-74612-0},
	MRCLASS = {18-02 (18A40 18D60 18D70 18M60)},
	MRNUMBER = {4274071},
	MRREVIEWER = {Nicola Gambino},
	DOI = {10.1017/9781108778657},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1017/9781108778657},
}

@misc{nlab:co-yoneda_lemma,
	author = {{nLab authors}},
	title = {co-{{Y}}oneda lemma},
	howpublished = {\url{https://ncatlab.org/nlab/show/co-Yoneda+lemma}},
	note = {\href{https://ncatlab.org/nlab/revision/co-Yoneda+lemma/21}{Revision 21}},
	month = feb,
	year = 2023
}

@article {dold,
	AUTHOR = {Dold, Albrecht},
	TITLE = {Homology of symmetric products and other functors of
		complexes},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {68},
	YEAR = {1958},
	PAGES = {54--80},
	ISSN = {0003-486X},
	MRCLASS = {55.00},
	MRNUMBER = {97057},
	MRREVIEWER = {Sze-tsen Hu},
	DOI = {10.2307/1970043},
	URL = {https://doi-org.pros1.lib.unimi.it/10.2307/1970043},
}

@article {transferredmodel,
	AUTHOR = {Crans, Sjoerd E.},
	TITLE = {Quillen closed model structures for sheaves},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {101},
	YEAR = {1995},
	NUMBER = {1},
	PAGES = {35--57},
	ISSN = {0022-4049},
	MRCLASS = {18D15 (18F20)},
	MRNUMBER = {1346427},
	DOI = {10.1016/0022-4049(94)00033-F},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/0022-4049(94)00033-F},
}

@MISC {cdgamodel,
	TITLE = {Non-examples of model structures, that fail for subtle/surprising reasons?},
	AUTHOR = {Tyler (https://mathoverflow.net/users/360/tyler-lawson), Lawson},
	HOWPUBLISHED = {MathOverflow},
%	NOTE = {URL:https://mathoverflow.net/q/23885 (version: 2012-05-08)},
	EPRINT = {https://mathoverflow.net/q/23885},
	URL = {https://mathoverflow.net/q/23885}
}

@article {duggeruniversalhomotopy,
	AUTHOR = {Dugger, Daniel},
	TITLE = {Universal homotopy theories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {164},
	YEAR = {2001},
	NUMBER = {1},
	PAGES = {144--176},
	ISSN = {0001-8708},
	MRCLASS = {18G55 (18E20 55U10)},
	MRNUMBER = {1870515},
	MRREVIEWER = {Manuel Bullejos Lorenzo},
	DOI = {10.1006/aima.2001.2014},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1006/aima.2001.2014},
}

@article {kan,
	AUTHOR = {Kan, Daniel M.},
	TITLE = {Functors involving c.s.s. complexes},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {87},
	YEAR = {1958},
	PAGES = {330--346},
	ISSN = {0002-9947},
	MRCLASS = {55.25},
	MRNUMBER = {131873},
	MRREVIEWER = {D. Puppe},
	DOI = {10.2307/1993103},
	URL = {https://doi-org.pros1.lib.unimi.it/10.2307/1993103},
}

@inproceedings{Dugger2009SHEAVESAH,
  title={SHEAVES AND HOMOTOPY THEORY},
  author={Daniel Dugger},
  year={2009},
  url={https://api.semanticscholar.org/CorpusID:17532173}
}

@book {saunders,
	AUTHOR = {MacLane, Saunders},
	TITLE = {Categories for the working mathematician},
	SERIES = {Graduate Texts in Mathematics, Vol. 5},
	PUBLISHER = {Springer-Verlag, New York-Berlin},
	YEAR = {1971},
	PAGES = {ix+262},
	MRCLASS = {18-02},
	MRNUMBER = {0354798},
	MRREVIEWER = {H.-B. Brinkmann},
}

@article {unboundedchain,
	AUTHOR = {Barthel, Tobias and May, J. P. and Riehl, Emily},
	TITLE = {Six model structures for {DG}-modules over {DGA}s: model
		category theory in homological action},
	JOURNAL = {New York J. Math.},
	FJOURNAL = {New York Journal of Mathematics},
	VOLUME = {20},
	YEAR = {2014},
	PAGES = {1077--1159},
	MRCLASS = {16E45 (18G55)},
	MRNUMBER = {3291613},
	MRREVIEWER = {Andrea Solotar},
	URL = {http://p8000-nyjm.albany.edu.pros1.lib.unimi.it/j/2014/20_1077.html},
}

@article {strom,
    AUTHOR = {Str\o m, Arne},
     TITLE = {The homotopy category is a homotopy category},
   JOURNAL = {Arch. Math. (Basel)},
  FJOURNAL = {Archiv der Mathematik},
    VOLUME = {23},
      YEAR = {1972},
     PAGES = {435--441},
      ISSN = {0003-889X,1420-8938},
   MRCLASS = {55F05},
  MRNUMBER = {321082},
MRREVIEWER = {A.\ K.\ Bousfield},
       DOI = {10.1007/BF01304912},
       URL = {https://doi.org/10.1007/BF01304912},
}

@book {quillenhomotopicalalgebra,
	AUTHOR = {Quillen, Daniel G.},
	TITLE = {Homotopical algebra},
	SERIES = {Lecture Notes in Mathematics, No. 43},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1967},
	PAGES = {iv+156 pp. (not consecutively paged)},
	MRCLASS = {18.20 (55.00)},
	MRNUMBER = {0223432},
	MRREVIEWER = {A. K. Bousfield},
}


@book {MR0420609,
	AUTHOR = {Boardman, J. M. and Vogt, R. M.},
	TITLE = {Homotopy invariant algebraic structures on topological spaces},
	SERIES = {Lecture Notes in Mathematics, Vol. 347},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1973},
	PAGES = {x+257},
	MRCLASS = {55D35},
	MRNUMBER = {0420609},
	MRREVIEWER = {J. Stasheff},
}


@article {rezk,
	AUTHOR = {Rezk, Charles},
	TITLE = {A model for the homotopy theory of homotopy theory},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {353},
	YEAR = {2001},
	NUMBER = {3},
	PAGES = {973--1007},
	ISSN = {0002-9947},
	MRCLASS = {55U35 (18G30)},
	MRNUMBER = {1804411},
	MRREVIEWER = {Brooke E. Shipley},
	DOI = {10.1090/S0002-9947-00-02653-2},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1090/S0002-9947-00-02653-2},
}


@article {albrechtpuppe,
	AUTHOR = {Dold, Albrecht and Puppe, Dieter},
	TITLE = {Homologie nicht-additiver {F}unktoren. {A}nwendungen},
	JOURNAL = {Ann. Inst. Fourier (Grenoble)},
	FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
	VOLUME = {11},
	YEAR = {1961},
	PAGES = {201--312},
	ISSN = {0373-0956},
	MRCLASS = {18.20},
	MRNUMBER = {150183},
	MRREVIEWER = {P. J. Hilton},
	URL = {http://www.numdam.org/item?id=AIF_1961__11__201_0},
}


@article {nuiten19,
	AUTHOR = {Nuiten, Joost},
	TITLE = {Homotopical algebra for {L}ie algebroids},
	JOURNAL = {Appl. Categ. Structures},
	FJOURNAL = {Applied Categorical Structures. A Journal Devoted to
		Applications of Categorical Methods in Algebra, Analysis,
		Order, Topology and Computer Science},
	VOLUME = {27},
	YEAR = {2019},
	NUMBER = {5},
	PAGES = {493--534},
	ISSN = {0927-2852},
	MRCLASS = {18G55 (55U15 55U35)},
	MRNUMBER = {4003715},
	MRREVIEWER = {Hirokazu Nishimura},
	DOI = {10.1007/s10485-019-09563-z},
	URL = {https://doi-org.pros2.lib.unimi.it/10.1007/s10485-019-09563-z},
}


@article {BMS,
    AUTHOR = {Bhatt, Bhargav and Morrow, Matthew and Scholze, Peter},
     TITLE = {Topological {H}ochschild homology and integral {$p$}-adic
              {H}odge theory},
   JOURNAL = {Publ. Math. Inst. Hautes \'{E}tudes Sci.},
  FJOURNAL = {Publications Math\'{e}matiques. Institut de Hautes \'{E}tudes
              Scientifiques},
    VOLUME = {129},
      YEAR = {2019},
     PAGES = {199--310},
      ISSN = {0073-8301},
   MRCLASS = {14F30 (13A35)},
  MRNUMBER = {3949030},
       DOI = {10.1007/s10240-019-00106-9},
       URL = {https://doi-org.pros.lib.unimi.it:2050/10.1007/s10240-019-00106-9},
}


@article {integraltransforms,
    AUTHOR = {Ben-Zvi, David and Francis, John and Nadler, David},
     TITLE = {Integral transforms and {D}rinfeld centers in derived
              algebraic geometry},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {23},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {909--966},
      ISSN = {0894-0347,1088-6834},
   MRCLASS = {14D23 (14F05 18D10 18E30)},
  MRNUMBER = {2669705},
MRREVIEWER = {Andrei\ D.\ Halanay},
       DOI = {10.1090/S0894-0347-10-00669-7},
       URL = {https://doi.org/10.1090/S0894-0347-10-00669-7},
}


@article {indcoh,
    AUTHOR = {Gaitsgory, Dennis},
     TITLE = {ind-coherent sheaves},
   JOURNAL = {Mosc. Math. J.},
  FJOURNAL = {Moscow Mathematical Journal},
    VOLUME = {13},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {399--528, 553},
      ISSN = {1609-3321},
   MRCLASS = {14F05 (14D24)},
  MRNUMBER = {3136100},
MRREVIEWER = {Cristian V. Anghel},
       DOI = {10.17323/1609-4514-2013-13-3-399-528},
       URL = {https://doi.org/10.17323/1609-4514-2013-13-3-399-528},
}


@book {serre,
	AUTHOR = {Serre, Jean-Pierre},
	TITLE = {Alg\`ebre locale. {M}ultiplicit\'{e}s},
	SERIES = {Lecture Notes in Mathematics},
	VOLUME = {11},
	NOTE = {Cours au Coll\`ege de France, 1957--1958, r\'{e}dig\'{e} par Pierre
		Gabriel,
		Seconde \'{e}dition, 1965},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1965},
	PAGES = {vii+188 pp. (not consecutively paged)},
	MRCLASS = {13.95 (14.08)},
	MRNUMBER = {0201468},
	MRREVIEWER = {M. Nagata},
}


@misc{UHKR,
    title={A Universal HKR Theorem},
    author={Tasos Moulinos and Marco Robalo and Bertrand Toën},
    year={2019},
    eprint={1906.00118},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}


@article {thetaspace,
    AUTHOR = {Rezk, Charles},
     TITLE = {A {C}artesian presentation of weak {$n$}-categories},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {14},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {521--571},
      ISSN = {1465-3060},
   MRCLASS = {18D05 (55U40)},
  MRNUMBER = {2578310},
       DOI = {10.2140/gt.2010.14.521},
       URL = {https://doi.org/10.2140/gt.2010.14.521},
}


@misc{enrichment,
  doi = {10.48550/ARXIV.2009.02428},
    url = {https://arxiv.org/abs/2009.02428},
    author = {Heine, Hadrian},
    keywords = {Algebraic Topology (math.AT), Category Theory (math.CT), FOS: Mathematics, FOS: Mathematics},
    title = {An equivalence between enriched $\infty$-categories and $\infty$-categories with weak action},
    publisher = {arXiv},
    year = {2020},
    copyright = {arXiv.org perpetual, non-exclusive license}
}


@article {thetaspaceerr,
    AUTHOR = {Rezk, Charles},
     TITLE = {Correction to ``{A} {C}artesian presentation of weak
              {$n$}-categories''},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {14},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {2301--2304},
      ISSN = {1465-3060,1364-0380},
   MRCLASS = {18D05 (55U40)},
  MRNUMBER = {2740648},
       DOI = {10.2140/gt.2010.14.2301},
       URL = {https://doi.org/10.2140/gt.2010.14.2301},
}


@article {kellerhochschildhomology,
    AUTHOR = {Keller, Bernhard},
     TITLE = {On the cyclic homology of ringed spaces and schemes},
   JOURNAL = {Doc. Math.},
  FJOURNAL = {Documenta Mathematica},
    VOLUME = {3},
      YEAR = {1998},
     PAGES = {231--259},
      ISSN = {1431-0635},
   MRCLASS = {16E40 (14F05 18E30)},
  MRNUMBER = {1647519},
MRREVIEWER = {Kevin P. Knudson},
}


@incollection {preygel,
    AUTHOR = {Preygel, Anatoly},
     TITLE = {Ind-coherent complexes on loop spaces and connections},
 BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
    SERIES = {Contemp. Math.},
    VOLUME = {643},
     PAGES = {289--323},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2015},
   MRCLASS = {14F05 (14F10 14F40)},
  MRNUMBER = {3381476},
MRREVIEWER = {Andreas H\"{o}ring},
       DOI = {10.1090/conm/643/12902},
       URL = {https://doi.org/10.1090/conm/643/12902},
}


@incollection {simpson,
    AUTHOR = {Simpson, Carlos},
     TITLE = {The {H}odge filtration on nonabelian cohomology},
 BOOKTITLE = {Algebraic geometry---{S}anta {C}ruz 1995},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {62},
     PAGES = {217--281},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1997},
   MRCLASS = {14F99 (14C30 14D20 32J25 32J27 53C55)},
  MRNUMBER = {1492538},
MRREVIEWER = {Nitin Nitsure},
       DOI = {10.1090/pspum/062.2/1492538},
       URL = {https://doi.org/10.1090/pspum/062.2/1492538},
}


@misc{benzvi2012morita,
      title={Morita equivalence for convolution categories: Appendix to arXiv:0805.0157}, 
      author={David Ben-Zvi and John Francis and David Nadler},
      year={2012},
      eprint={1209.0193},
      archivePrefix={arXiv},
      primaryClass={math.AG}
}


@article {BZN,
    AUTHOR = {Ben-Zvi, David and Nadler, David},
     TITLE = {Loop spaces and connections},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {5},
      YEAR = {2012},
    NUMBER = {2},
     PAGES = {377--430},
      ISSN = {1753-8416},
   MRCLASS = {14F05 (14F10 19D55 55P35)},
  MRNUMBER = {2928082},
MRREVIEWER = {Julia Bergner},
       DOI = {10.1112/jtopol/jts007},
       URL = {https://doi.org/10.1112/jtopol/jts007},
}


@article {HKRTV,
    AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
     TITLE = {Alg\`ebres simpliciales {$S^1$}-\'{e}quivariantes, th\'{e}orie de de
              {R}ham et th\'{e}or\`emes {HKR} multiplicatifs},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {147},
      YEAR = {2011},
    NUMBER = {6},
     PAGES = {1979--2000},
      ISSN = {0010-437X},
   MRCLASS = {18G55 (14F40 16E45 18G30 55U10)},
  MRNUMBER = {2862069},
MRREVIEWER = {Kenneth A. Brown},
       DOI = {10.1112/S0010437X11005501},
       URL = {https://doi.org/10.1112/S0010437X11005501},
}


@incollection {gwtheory,
    AUTHOR = {Rose, Simon C. F.},
     TITLE = {Introduction to {G}romov-{W}itten theory},
 BOOKTITLE = {Calabi-{Y}au varieties: arithmetic, geometry and physics},
    SERIES = {Fields Inst. Monogr.},
    VOLUME = {34},
     PAGES = {281--301},
 PUBLISHER = {Fields Inst. Res. Math. Sci., Toronto, ON},
      YEAR = {2015},
   MRCLASS = {14N35 (53D45)},
  MRNUMBER = {3409778},
MRREVIEWER = {Hsian-Hua Tseng},
       DOI = {10.1007/978-1-4939-2830-9_8},
       URL = {https://doi.org/10.1007/978-1-4939-2830-9_8},
}




@misc{hoyois2018categorified,
    title={The categorified Grothendieck-Riemann-Roch theorem},
    author={Marc Hoyois and Pavel Safronov and Sarah Scherotzke and Nicolò Sibilla},
    year={2018},
    eprint={1804.00879},
    archivePrefix={arXiv},
    primaryClass={math.KT}
}


@article {GR,
    AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
     TITLE = {Crystals and {D}-modules},
   JOURNAL = {Pure Appl. Math. Q.},
  FJOURNAL = {Pure and Applied Mathematics Quarterly},
    VOLUME = {10},
      YEAR = {2014},
    NUMBER = {1},
     PAGES = {57--154},
      ISSN = {1558-8599},
   MRCLASS = {14A20 (14F05 14F10)},
  MRNUMBER = {3264953},
MRREVIEWER = {Andrei D. Halanay},
       DOI = {10.4310/PAMQ.2014.v10.n1.a2},
       URL = {https://doi.org/10.4310/PAMQ.2014.v10.n1.a2},
}


@article {barannikov,
    AUTHOR = {Barannikov, Serguei},
     TITLE = {Quantum periods. {I}. {S}emi-infinite variations of {H}odge
              structures},
   JOURNAL = {Internat. Math. Res. Notices},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {2001},
    NUMBER = {23},
     PAGES = {1243--1264},
      ISSN = {1073-7928},
   MRCLASS = {32G20 (14D07 14J32 32J25 32Q25)},
  MRNUMBER = {1866443},
MRREVIEWER = {Gregory J. Pearlstein},
       DOI = {10.1155/S1073792801000599},
       URL = {https://doi.org/10.1155/S1073792801000599},
}


@article {mukaipairing,
    AUTHOR = {C\u{a}ld\u{a}raru, Andrei},
     TITLE = {The {M}ukai pairing. {II}. {T}he
              {H}ochschild-{K}ostant-{R}osenberg isomorphism},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {194},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {34--66},
      ISSN = {0001-8708},
   MRCLASS = {14F40 (19L10)},
  MRNUMBER = {2141853},
MRREVIEWER = {David Ploog},
       DOI = {10.1016/j.aim.2004.05.012},
       URL = {https://doi.org/10.1016/j.aim.2004.05.012},
}


@misc{sheridanncht,
    title={Formulae in noncommutative Hodge theory},
    author={Nick Sheridan},
    year={2015},
    eprint={1510.03795},
    archivePrefix={arXiv},
    primaryClass={math.KT}
}


@article {GMconnection,
    AUTHOR = {Katz, Nicholas M. and Oda, Tadao},
     TITLE = {On the differentiation of de {R}ham cohomology classes with
              respect to parameters},
   JOURNAL = {J. Math. Kyoto Univ.},
  FJOURNAL = {Journal of Mathematics of Kyoto University},
    VOLUME = {8},
      YEAR = {1968},
     PAGES = {199--213},
      ISSN = {0023-608X},
   MRCLASS = {14.52},
  MRNUMBER = {237510},
MRREVIEWER = {James Milne},
       DOI = {10.1215/kjm/1250524135},
       URL = {https://doi.org/10.1215/kjm/1250524135},
}


@article {shklyarov,
    AUTHOR = {Shklyarov, Dmytro},
     TITLE = {Matrix factorizations and higher residue pairings},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {292},
      YEAR = {2016},
     PAGES = {181--209},
      ISSN = {0001-8708},
   MRCLASS = {14A22 (16E40 16E45 18D10 32S50)},
  MRNUMBER = {3464022},
MRREVIEWER = {Andrea Solotar},
       DOI = {10.1016/j.aim.2016.01.014},
       URL = {https://doi.org/10.1016/j.aim.2016.01.014},
}

@misc{raksit2020,
      title={Hochschild homology and the derived de Rham complex revisited}, 
      author={Arpon Raksit},
      year={2020},
      eprint={2007.02576},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2007.02576}, 
}

@incollection {getzler,
    AUTHOR = {Getzler, Ezra},
     TITLE = {Cartan homotopy formulas and the {G}auss-{M}anin connection in
              cyclic homology},
 BOOKTITLE = {Quantum deformations of algebras and their representations
              ({R}amat-{G}an, 1991/1992; {R}ehovot, 1991/1992)},
    SERIES = {Israel Math. Conf. Proc.},
    VOLUME = {7},
     PAGES = {65--78},
 PUBLISHER = {Bar-Ilan Univ., Ramat Gan},
      YEAR = {1993},
   MRCLASS = {19D55 (18G60 53C05)},
  MRNUMBER = {1261901},
MRREVIEWER = {Ulrike Tillmann},
}


@article {highertraces,
	AUTHOR = {Hoyois, Marc and Scherotzke, Sarah and Sibilla, Nicol\`o},
	TITLE = {Higher traces, noncommutative motives, and the categorified
		{C}hern character},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {309},
	YEAR = {2017},
	PAGES = {97--154},
	ISSN = {0001-8708},
	MRCLASS = {14F05 (14F42 18D05 19D55)},
	MRNUMBER = {3607274},
	MRREVIEWER = {Satoshi Mochizuki},
	DOI = {10.1016/j.aim.2017.01.008},
	URL = {https://doi.org/10.1016/j.aim.2017.01.008},
}


@article {eilenbergmoorespectralsequence,
	AUTHOR = {Eilenberg, Samuel and Moore, John C.},
	TITLE = {Homology and fibrations. {I}. {C}oalgebras, cotensor product
		and its derived functors},
	JOURNAL = {Comment. Math. Helv.},
	FJOURNAL = {Commentarii Mathematici Helvetici},
	VOLUME = {40},
	YEAR = {1966},
	PAGES = {199--236},
	ISSN = {0010-2571},
	MRCLASS = {55.50},
	MRNUMBER = {203730},
	MRREVIEWER = {A. Heller},
	DOI = {10.1007/BF02564371},
	URL = {https://doi.org/10.1007/BF02564371},
}


@article {koszuldualitypatterns,
	AUTHOR = {Beilinson, Alexander and Ginzburg, Victor and Soergel,
		Wolfgang},
	TITLE = {Koszul duality patterns in representation theory},
	JOURNAL = {J. Amer. Math. Soc.},
	FJOURNAL = {Journal of the American Mathematical Society},
	VOLUME = {9},
	YEAR = {1996},
	NUMBER = {2},
	PAGES = {473--527},
	ISSN = {0894-0347},
	MRCLASS = {17B10 (14F10 16W50)},
	MRNUMBER = {1322847},
	MRREVIEWER = {Rolf K\"{a}llstr\"{o}m},
	DOI = {10.1090/S0894-0347-96-00192-0},
	URL = {https://doi.org/10.1090/S0894-0347-96-00192-0},
}


@article {arinkingaitsgory,
	AUTHOR = {Arinkin, D. and Gaitsgory, D.},
	TITLE = {Singular support of coherent sheaves and the geometric
		{L}anglands conjecture},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {21},
	YEAR = {2015},
	NUMBER = {1},
	PAGES = {1--199},
	ISSN = {1022-1824},
	MRCLASS = {14D24 (14A20 14F05 22E57)},
	MRNUMBER = {3300415},
	MRREVIEWER = {Richard P. Thomas},
	DOI = {10.1007/s00029-014-0167-5},
	URL = {https://doi.org/10.1007/s00029-014-0167-5},
}


@article {haineportateyssier,
    AUTHOR = {Haine, Peter J. and Porta, Mauro and Teyssier, Jean-Baptiste},
     TITLE = {The homotopy-invariance of constructible sheaves},
   JOURNAL = {Homology Homotopy Appl.},
  FJOURNAL = {Homology, Homotopy and Applications},
    VOLUME = {25},
      YEAR = {2023},
    NUMBER = {2},
     PAGES = {97--128},
      ISSN = {1532-0073,1532-0081},
   MRCLASS = {55N30 (18F20 32S60 55N05 55P55)},
  MRNUMBER = {4651175},
       DOI = {10.4310/hha.2023.v25.n2.a6},
       URL = {https://doi.org/10.4310/hha.2023.v25.n2.a6},
}


@misc{symmetricspectra,
AUTHOR = {Schwede, Stefan},
TITLE = {Symmetric Spectra},
YEAR = {2012},
URL ={http://www.math.uni-bonn.de/people/schwede/SymSpec-v3.pdf}
}

@misc{khan_notes,
AUTHOR = {Khan, Adeel A.},
TITLE = {An introduction to derived algebraic geometry},
YEAR={2023},
URL={https://www.preschema.com/lecture-notes/2023-kias/dagkias.pdf}
}

@article {dwyerduality,
	AUTHOR = {Dwyer, W. G. and Greenlees, J. P. C. and Iyengar, S.},
	TITLE = {Duality in algebra and topology},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {200},
	YEAR = {2006},
	NUMBER = {2},
	PAGES = {357--402},
	ISSN = {0001-8708},
	MRCLASS = {55P43 (13H10 16D90 18E30 55R40 57N65)},
	MRNUMBER = {2200850},
	MRREVIEWER = {Andrey Yu. Lazarev},
	DOI = {10.1016/j.aim.2005.11.004},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/j.aim.2005.11.004},
}


@article {rothenbergsteenrod,
	AUTHOR = {Rothenberg, M. and Steenrod, N. E.},
	TITLE = {The cohomology of classifying spaces of {$H$}-spaces},
	JOURNAL = {Bull. Amer. Math. Soc.},
	FJOURNAL = {Bulletin of the American Mathematical Society},
	VOLUME = {71},
	YEAR = {1965},
	PAGES = {872--875},
	ISSN = {0002-9904},
	MRCLASS = {55.40},
	MRNUMBER = {208596},
	MRREVIEWER = {A. Dold},
	DOI = {10.1090/S0002-9904-1965-11420-3},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1090/S0002-9904-1965-11420-3},
}


@incollection {perversesheaves,
	AUTHOR = {Be\u{\i}linson, A. A. and Bernstein, J. and Deligne, P.},
	TITLE = {Faisceaux pervers},
	BOOKTITLE = {Analysis and topology on singular spaces, {I} ({L}uminy,
		1981)},
	SERIES = {Ast\'{e}risque},
	VOLUME = {100},
	PAGES = {5--171},
	PUBLISHER = {Soc. Math. France, Paris},
	YEAR = {1982},
	MRCLASS = {32C38},
	MRNUMBER = {751966},
	MRREVIEWER = {Zoghman Mebkhout},
}


@book {mccleary,
    AUTHOR = {McCleary, John},
     TITLE = {A user's guide to spectral sequences},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {58},
   EDITION = {Second},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2001},
     PAGES = {xvi+561},
      ISBN = {0-521-56759-9},
   MRCLASS = {55Txx (18G40)},
  MRNUMBER = {1793722},
MRREVIEWER = {Frank\ Neumann},
}


@incollection {1affineness,
	AUTHOR = {Gaitsgory, Dennis},
	TITLE = {Sheaves of categories and the notion of 1-affineness},
	BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
	SERIES = {Contemp. Math.},
	VOLUME = {643},
	PAGES = {127--225},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {2015},
	MRCLASS = {14F05 (14A20)},
	MRNUMBER = {3381473},
	MRREVIEWER = {Jon Eivind Vatne},
	DOI = {10.1090/conm/643/12899},
	URL = {https://doi.org/10.1090/conm/643/12899},
}


@article {beke,
	AUTHOR = {Beke, Tibor},
	TITLE = {Sheafifiable homotopy model categories},
	JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
	FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
		Society},
	VOLUME = {129},
	YEAR = {2000},
	NUMBER = {3},
	PAGES = {447--475},
	ISSN = {0305-0041},
	MRCLASS = {18D15 (03C95 18F20 18G55)},
	MRNUMBER = {1780498},
	MRREVIEWER = {Masahiko Niwa},
	DOI = {10.1017/S0305004100004722},
	URL = {https://doi.org/10.1017/S0305004100004722},
}


@misc{stefanich2020presentable,
	title={Presentable $(\infty, n)$-categories}, 
	author={Germán Stefanich},
	year={2020},
	eprint={2011.03035},
	archivePrefix={arXiv},
	primaryClass={math.AT}
}
@book {stefanichthesis,
    AUTHOR = {Stefanich, German},
     TITLE = {Higher {Q}uasicoherent {S}heaves},
      NOTE = {Thesis (Ph.D.)--University of California, Berkeley},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2021},
     PAGES = {347},
      ISBN = {979-8535-56467-8},
   MRCLASS = {99-05},
  MRNUMBER = {4326588},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:28540389},
}


@article {iwanari,
	AUTHOR = {Iwanari, Isamu},
	TITLE = {Differential calculus of {H}ochschild pairs for
		infinity-categories},
	JOURNAL = {SIGMA Symmetry Integrability Geom. Methods Appl.},
	FJOURNAL = {SIGMA. Symmetry, Integrability and Geometry. Methods and
		Applications},
	VOLUME = {16},
	YEAR = {2020},
	PAGES = {Paper No. 097, 57},
	MRCLASS = {16E40 (18M60 18N60)},
	MRNUMBER = {4156865},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.3842/SIGMA.2020.097},
	URL = {https://doi.org/10.3842/SIGMA.2020.097},
}


@article {schwedeshipley,
	AUTHOR = {Schwede, Stefan and Shipley, Brooke E.},
	TITLE = {Algebras and modules in monoidal model categories},
	JOURNAL = {Proc. London Math. Soc. (3)},
	FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
	VOLUME = {80},
	YEAR = {2000},
	NUMBER = {2},
	PAGES = {491--511},
	ISSN = {0024-6115},
	MRCLASS = {18D10 (18D50 55P48 55U35)},
	MRNUMBER = {1734325},
	MRREVIEWER = {Mark Hovey},
	DOI = {10.1112/S002461150001220X},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/S002461150001220X},
}


@article {aciclicitythm,
	AUTHOR = {Hess, Kathryn and K\c{e}dziorek, Magdalena and Riehl, Emily and
		Shipley, Brooke},
	TITLE = {A necessary and sufficient condition for induced model
		structures},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {10},
	YEAR = {2017},
	NUMBER = {2},
	PAGES = {324--369},
	ISSN = {1753-8416},
	MRCLASS = {55U35 (18G55)},
	MRNUMBER = {3653314},
	MRREVIEWER = {J\'{e}r\^{o}me Scherer},
	DOI = {10.1112/topo.12011},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/topo.12011},
}


@article {hovey2,
	AUTHOR = {Hovey, Mark},
	TITLE = {Model category structures on chain complexes of sheaves},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {353},
	YEAR = {2001},
	NUMBER = {6},
	PAGES = {2441--2457},
	ISSN = {0002-9947},
	MRCLASS = {18F20 (14F05 18E15 18E30 55U35)},
	MRNUMBER = {1814077},
	MRREVIEWER = {J. F. Jardine},
	DOI = {10.1090/S0002-9947-01-02721-0},
	URL = {https://doi.org/10.1090/S0002-9947-01-02721-0},
}


@article {shipley,
	AUTHOR = {Shipley, Brooke},
	TITLE = {{$H\Bbb Z$}-algebra spectra are differential graded algebras},
	JOURNAL = {Amer. J. Math.},
	FJOURNAL = {American Journal of Mathematics},
	VOLUME = {129},
	YEAR = {2007},
	NUMBER = {2},
	PAGES = {351--379},
	ISSN = {0002-9327},
	MRCLASS = {55P42 (18G55 55P20 55P43 55U35)},
	MRNUMBER = {2306038},
	MRREVIEWER = {Tyler D. Lawson},
	DOI = {10.1353/ajm.2007.0014},
	URL = {https://doi.org/10.1353/ajm.2007.0014},
}


@article {toenchampsaffines,
    AUTHOR = {To\"{e}n, Bertrand},
     TITLE = {Champs affines},
   JOURNAL = {Selecta Math. (N.S.)},
  FJOURNAL = {Selecta Mathematica. New Series},
    VOLUME = {12},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {39--135},
      ISSN = {1022-1824,1420-9020},
   MRCLASS = {14F35 (14A20 18F10 55U35)},
  MRNUMBER = {2244263},
MRREVIEWER = {Mark\ Hovey},
       DOI = {10.1007/s00029-006-0019-z},
       URL = {https://doi.org/10.1007/s00029-006-0019-z},
}


@book {hovey,
	AUTHOR = {Hovey, Mark},
	TITLE = {Model categories},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {63},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {1999},
	PAGES = {xii+209},
	ISBN = {0-8218-1359-5},
	MRCLASS = {55U35 (18D15 18G30 18G55)},
	MRNUMBER = {1650134},
	MRREVIEWER = {Teimuraz Pirashvili},
}


@misc{pantev2021moduli,
	title={Moduli of flat connections on smooth varieties}, 
	author={Tony Pantev and Bertrand Toën},
	year={2021},
	eprint={1905.12124},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@incollection {KSmirrorsymmetry,
	AUTHOR = {Kontsevich, Maxim and Soibelman, Yan},
	TITLE = {Homological mirror symmetry and torus fibrations},
	BOOKTITLE = {Symplectic geometry and mirror symmetry ({S}eoul, 2000)},
	PAGES = {203--263},
	PUBLISHER = {World Sci. Publ., River Edge, NJ},
	YEAR = {2001},
	MRCLASS = {32Q25 (14J32 14K05 18E30 32G05 53C38)},
	MRNUMBER = {1882331},
	MRREVIEWER = {Bal\'{a}zs Szendr\H{o}i},
	DOI = {10.1142/9789812799821_0007},
	URL = {https://doi.org/10.1142/9789812799821_0007},
}


@incollection {beilinsonderived,
    AUTHOR = {Beilinson, A. A.},
     TITLE = {On the derived category of perverse sheaves},
 BOOKTITLE = {{$K$}-theory, arithmetic and geometry ({M}oscow, 1984--1986)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1289},
     PAGES = {27--41},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1987},
   MRCLASS = {14F99 (18E30 18F20 32C38 58G07)},
  MRNUMBER = {923133},
MRREVIEWER = {Jean-Luc Brylinski},
       DOI = {10.1007/BFb0078365},
       URL = {https://doi-org.pros.lib.unimi.it:2050/10.1007/BFb0078365},
}
		


@article {beilinsonadic,
	AUTHOR = {Beilinson, A.},
	TITLE = {{$p$}-adic periods and derived de {R}ham cohomology},
	JOURNAL = {J. Amer. Math. Soc.},
	FJOURNAL = {Journal of the American Mathematical Society},
	VOLUME = {25},
	YEAR = {2012},
	NUMBER = {3},
	PAGES = {715--738},
	ISSN = {0894-0347},
	MRCLASS = {14F40 (14F20 14F30 16E45)},
	MRNUMBER = {2904571},
	MRREVIEWER = {Nobuo Tsuzuki},
	DOI = {10.1090/S0894-0347-2012-00729-2},
	URL = {https://doi.org/10.1090/S0894-0347-2012-00729-2},
}




@incollection {lurieelliptic,
	AUTHOR = {Lurie, J.},
	TITLE = {A survey of elliptic cohomology},
	BOOKTITLE = {Algebraic topology},
	SERIES = {Abel Symp.},
	VOLUME = {4},
	PAGES = {219--277},
	PUBLISHER = {Springer, Berlin},
	YEAR = {2009},
	MRCLASS = {55N34 (55P43)},
	MRNUMBER = {2597740},
	MRREVIEWER = {Tyler D. Lawson},
	DOI = {10.1007/978-3-642-01200-6_9},
	URL = {https://doi.org/10.1007/978-3-642-01200-6_9},
}


@book {illusie,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {I}},
	SERIES = {Lecture Notes in Mathematics, Vol. 239},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1971},
	PAGES = {xv+355},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491680},
	MRREVIEWER = {Larry Breen},
}


@inproceedings {quillenhomology,
	AUTHOR = {Quillen, Daniel},
	TITLE = {On the (co-) homology of commutative rings},
	BOOKTITLE = {Applications of {C}ategorical {A}lgebra ({P}roc. {S}ympos.
		{P}ure {M}ath., {V}ol. {XVII}, {N}ew {Y}ork, 1968)},
	PAGES = {65--87},
	PUBLISHER = {Amer. Math. Soc., Providence, R.I.},
	YEAR = {1970},
	MRCLASS = {13.90 (18.00)},
	MRNUMBER = {0257068},
	MRREVIEWER = {S. Yuan},
}

@article {COS,
	AUTHOR = {Canonaco, Alberto and Ornaghi, Mattia and Stellari, Paolo},
	TITLE = {Localizations of the category of {$A_\infty$} categories and
		internal {H}oms},
	JOURNAL = {Doc. Math.},
	FJOURNAL = {Documenta Mathematica},
	VOLUME = {24},
	YEAR = {2019},
	PAGES = {2463--2492},
	ISSN = {1431-0635},
	MRCLASS = {18G80 (18D20 18G35 18G70 57T30)},
	MRNUMBER = {4061058},
	MRREVIEWER = {J\'{e}r\^{o}me Scherer},
}

@article{cohn,
	AUTHOR = {Cohn, Lee},
	TITLE={Differential graded categories are {$k$}-linear stable infinity categories},
	YEAR={2013},
	URL={arXiv:1308.2587},
}


@article {bravdyckerhoff2,
	AUTHOR = {Brav, Christopher and Dyckerhoff, Tobias},
	TITLE = {Relative {C}alabi-{Y}au structures {II}: shifted {L}agrangians
		in the moduli of objects},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {27},
	YEAR = {2021},
	NUMBER = {4},
	PAGES = {Paper No. 63, 45},
	ISSN = {1022-1824},
	MRCLASS = {14F08 (14D23 14J32 18G35 18G80 53C55)},
	MRNUMBER = {4281260},
	MRREVIEWER = {\Dbar \cftil{o} Ng\d{o}c Di\cfudot{e}p},
	DOI = {10.1007/s00029-021-00642-5},
	URL = {https://doi.org/10.1007/s00029-021-00642-5},
}




@book {loday,
	AUTHOR = {Loday, Jean-Louis},
	TITLE = {Cyclic homology},
	SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
		Principles of Mathematical Sciences]},
	VOLUME = {301},
	EDITION = {Second},
	NOTE = {Appendix E by Mar\'{\i}a O. Ronco,
		Chapter 13 by the author in collaboration with Teimuraz
		Pirashvili},
	PUBLISHER = {Springer-Verlag, Berlin},
	YEAR = {1998},
	PAGES = {xx+513},
	ISBN = {3-540-63074-0},
	MRCLASS = {16E40 (13D03 17B55 18G60 19D55)},
	MRNUMBER = {1600246},
	DOI = {10.1007/978-3-662-11389-9},
	URL = {https://doi.org/10.1007/978-3-662-11389-9},
}


@article {BGT,
	AUTHOR = {Blumberg, Andrew J. and Gepner, David and Tabuada, Gon\c{c}alo},
	TITLE = {A universal characterization of higher algebraic {$K$}-theory},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {17},
	YEAR = {2013},
	NUMBER = {2},
	PAGES = {733--838},
	ISSN = {1465-3060},
	MRCLASS = {19D10 (18D20 19D25 19D55 55N15 55U40)},
	MRNUMBER = {3070515},
	MRREVIEWER = {Ross Staffeldt},
	DOI = {10.2140/gt.2013.17.733},
	URL = {https://doi.org/10.2140/gt.2013.17.733},
}


@article {cyclichomology2,
	AUTHOR = {Keller, Bernhard},
	TITLE = {On the cyclic homology of ringed spaces and schemes},
	JOURNAL = {Doc. Math.},
	FJOURNAL = {Documenta Mathematica},
	VOLUME = {3},
	YEAR = {1998},
	PAGES = {231--259},
	ISSN = {1431-0635},
	MRCLASS = {16E40 (14F05 18E30)},
	MRNUMBER = {1647519},
	MRREVIEWER = {Kevin P. Knudson},
}


@article {orlov,
	AUTHOR = {Orlov, Dmitri},
	TITLE = {Smooth and proper noncommutative schemes and gluing of {DG}
		categories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {302},
	YEAR = {2016},
	PAGES = {59--105},
	ISSN = {0001-8708},
	MRCLASS = {14F05 (16E45 18E30)},
	MRNUMBER = {3545926},
	MRREVIEWER = {Shintarou Yanagida},
	DOI = {10.1016/j.aim.2016.07.014},
	URL = {https://doi.org/10.1016/j.aim.2016.07.014},
}


@article {keller2,
	AUTHOR = {Keller, Bernhard},
	TITLE = {Deriving {DG} categories},
	JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
	FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
		S\'{e}rie},
	VOLUME = {27},
	YEAR = {1994},
	NUMBER = {1},
	PAGES = {63--102},
	ISSN = {0012-9593},
	MRCLASS = {18E30 (16D90)},
	MRNUMBER = {1258406},
	MRREVIEWER = {Jeremy Rickard},
	URL = {http://www.numdam.org/item?id=ASENS_1994_4_27_1_63_0},
}


@article {hag1,
	AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
	TITLE = {Homotopical algebraic geometry. {I}. {T}opos theory},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {193},
	YEAR = {2005},
	NUMBER = {2},
	PAGES = {257--372},
	ISSN = {0001-8708},
	MRCLASS = {14F20 (18F20 18G55 55U40)},
	MRNUMBER = {2137288},
	MRREVIEWER = {Paul Arne \O stv\ae r},
	DOI = {10.1016/j.aim.2004.05.004},
	URL = {https://doi.org/10.1016/j.aim.2004.05.004},
}


@article {hag2,
	AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
	TITLE = {Homotopical algebraic geometry. {II}. {G}eometric stacks and
		applications},
	JOURNAL = {Mem. Amer. Math. Soc.},
	FJOURNAL = {Memoirs of the American Mathematical Society},
	VOLUME = {193},
	YEAR = {2008},
	NUMBER = {902},
	PAGES = {x+224},
	ISSN = {0065-9266},
	MRCLASS = {14A20 (18F10 18F20 18G55 55P42 55U40)},
	MRNUMBER = {2394633},
	MRREVIEWER = {Paul Arne \O stv\ae r},
	DOI = {10.1090/memo/0902},
	URL = {https://doi.org/10.1090/memo/0902},
}


@article{BCS,
	AUTHOR={Bozec, Tristan and Calaque, Damien and Scherotzke, Sarah},
	TITLE={Relative critical loci and quiver moduli},
	YEAR={2021},
	URL = {arXiv:2006.01069v2},
}


@article{robalo,
	AUTHOR={Robalo, Marco},
	TITLE={Noncommutative Motives I: A Universal Characterization of the Motivic Stable Homotopy Theory of Schemes},
	YEAR={2013},
	URL = {arXiv:1206.3645v3},
}


@article {keller,
	AUTHOR = {Keller, Bernhard},
	TITLE = {On the cyclic homology of exact categories},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {136},
	YEAR = {1999},
	NUMBER = {1},
	PAGES = {1--56},
	ISSN = {0022-4049},
	MRCLASS = {18G60 (18E10)},
	MRNUMBER = {1667558},
	MRREVIEWER = {Teimuraz Pirashvili},
	DOI = {10.1016/S0022-4049(97)00152-7},
	URL = {https://doi.org/10.1016/S0022-4049(97)00152-7},
}


@article {iteratedspans,
	AUTHOR = {Haugseng, Rune},
	TITLE = {Iterated spans and classical topological field theories},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {289},
	YEAR = {2018},
	NUMBER = {3-4},
	PAGES = {1427--1488},
	ISSN = {0025-5874},
	MRCLASS = {18D05 (14A20 14F05 81R10)},
	MRNUMBER = {3830256},
	DOI = {10.1007/s00209-017-2005-x},
	URL = {https://doi.org/10.1007/s00209-017-2005-x},
}


@article {igusa,
	AUTHOR = {Igusa, Jun-ichi},
	TITLE = {Fibre systems of {J}acobian varieties. {III}. {F}ibre systems
		of elliptic curves},
	JOURNAL = {Amer. J. Math.},
	FJOURNAL = {American Journal of Mathematics},
	VOLUME = {81},
	YEAR = {1959},
	PAGES = {453--476},
	ISSN = {0002-9327},
	MRCLASS = {14.00},
	MRNUMBER = {0104669},
	MRREVIEWER = {M. Rosenlicht},
	DOI = {10.2307/2372751},
	URL = {https://doi.org/10.2307/2372751},
}


@article {drinfeld,
	AUTHOR = {Drinfeld, V. G.},
	TITLE = {Elliptic modules},
	JOURNAL = {Mat. Sb. (N.S.)},
	VOLUME = {94(136)},
	YEAR = {1974},
	PAGES = {594--627, 656},
	MRCLASS = {10D99 (14K15)},
	MRNUMBER = {0384707},
	MRREVIEWER = {Pierre Deligne},
}


@article {DR,
	AUTHOR = {Deligne, P. and Rapoport, M.},
	TITLE = {Les sch\'{e}mas de modules de courbes elliptiques},
	BOOKTITLE = {Modular functions of one variable, {II} ({P}roc. {I}nternat.
		{S}ummer {S}chool, {U}niv. {A}ntwerp, {A}ntwerp, 1972)},
	PAGES = {143--316. Lecture Notes in Math., Vol. 349},
	PUBLISHER = {Springer, Berlin},
	YEAR = {1973},
	MRCLASS = {14K10 (10D05)},
	MRNUMBER = {0337993},
	MRREVIEWER = {T. Oda},
}


@book {KM,
	AUTHOR = {Katz, Nicholas M. and Mazur, Barry},
	TITLE = {Arithmetic moduli of elliptic curves},
	SERIES = {Annals of Mathematics Studies},
	VOLUME = {108},
	PUBLISHER = {Princeton University Press, Princeton, NJ},
	YEAR = {1985},
	PAGES = {xiv+514},
	ISBN = {0-691-08349-5; 0-691-08352-5},
	MRCLASS = {11G05 (11F11 14G25 14K15)},
	MRNUMBER = {772569},
	MRREVIEWER = {Kenneth A. Ribet},
	DOI = {10.1515/9781400881710},
	URL = {https://doi.org/10.1515/9781400881710},
}


@article{CPTVV,
	AUTHOR = {Calaque, Damien and Pantev, Tony and To\"{e}n, Bertrand and
		Vaqui\'{e}, Michel and Vezzosi, Gabriele},
	TITLE = {Shifted {P}oisson structures and deformation quantization},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {10},
	YEAR = {2017},
	NUMBER = {2},
	PAGES = {483--584},
	ISSN = {1753-8416},
	MRCLASS = {14A20 (14D15 14F05 18E30 18G55 53D55)},
	MRNUMBER = {3653319},
	MRREVIEWER = {Scott R. Nollet},
	DOI = {10.1112/topo.12012},
	URL = {https://doi.org/10.1112/topo.12012},
}

@book{1,
	author = {Mobilio, Settimio and Boscherini, Federico and Meneghini, C.},
	year = {2015},
	month = {01},
	pages = {1-799},
	title = {Synchrotron radiation: Basics, methods and applications},
	doi = {10.1007/978-3-642-55315-8}
}


@Misc{2,
	AUTHOR = {Barbarino, Sebastiano},
	TITLE = {Appunti di Campi Elettromagnetici},
	YEAR = {2013},
	URL = {http://www.diit.unict.it/users/campi/appunti_campi_indice.htm},
}


@misc{calaque2021lie,
	title={Lie algebroids are curved Lie algebras}, 
	author={Damien Calaque and Ricardo Campos and Joost Nuiten},
	year={2021},
	eprint={2103.10728},
	archivePrefix={arXiv},
	primaryClass={math.AT}
}


@article {PTVV,
AUTHOR = {Pantev, Tony and To\"{e}n, Bertrand and Vaqui\'{e}, Michel and
	Vezzosi, Gabriele},
TITLE = {Shifted symplectic structures},
JOURNAL = {Publ. Math. Inst. Hautes \'{E}tudes Sci.},
FJOURNAL = {Publications Math\'{e}matiques. Institut de Hautes \'{E}tudes
	Scientifiques},
VOLUME = {117},
YEAR = {2013},
PAGES = {271--328},
ISSN = {0073-8301},
MRCLASS = {14F05 (14A15 18F20 18G30 53D05 53D12)},
MRNUMBER = {3090262},
MRREVIEWER = {Andrey Yu. Lazarev},
DOI = {10.1007/s10240-013-0054-1},
URL = {https://doi.org/10.1007/s10240-013-0054-1},
}


@article {sullivanmodel,
    AUTHOR = {Sullivan, Dennis},
     TITLE = {Infinitesimal computations in topology},
   JOURNAL = {Inst. Hautes \'{E}tudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'{E}tudes Scientifiques. Publications
              Math\'{e}matiques},
    NUMBER = {47},
      YEAR = {1977},
     PAGES = {269--331},
      ISSN = {0073-8301,1618-1913},
   MRCLASS = {57D99 (55D99 58A10)},
  MRNUMBER = {646078},
MRREVIEWER = {J.\ F.\ Adams},
       URL = {http://www.numdam.org/item?id=PMIHES_1977__47__269_0},
}


@article {plderham,
    AUTHOR = {Bousfield, A. K. and Gugenheim, V. K. A. M.},
     TITLE = {On {${\rm PL}$} de {R}ham theory and rational homotopy type},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {8},
      YEAR = {1976},
    NUMBER = {179},
     PAGES = {ix+94},
      ISSN = {0065-9266,1947-6221},
   MRCLASS = {55D15 (58A10)},
  MRNUMBER = {425956},
MRREVIEWER = {Jean-Michel\ Lemaire},
       DOI = {10.1090/memo/0179},
       URL = {https://doi.org/10.1090/memo/0179},
}


@article {berglundkoszul,
    AUTHOR = {Berglund, Alexander},
     TITLE = {Koszul spaces},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {366},
      YEAR = {2014},
    NUMBER = {9},
     PAGES = {4551--4569},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {55P62 (16S37 18D50)},
  MRNUMBER = {3217692},
MRREVIEWER = {Samuel\ B.\ Smith},
       DOI = {10.1090/S0002-9947-2014-05935-7},
       URL = {https://doi.org/10.1090/S0002-9947-2014-05935-7},
}


@book {studyindag2,
	AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
	TITLE = {A study in derived algebraic geometry. {V}ol. {II}.
		{D}eformations, {L}ie theory and formal geometry},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {221},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2017},
	PAGES = {xxxv+436},
	ISBN = {978-1-4704-3570-7},
	MRCLASS = {14F05 (18D05 18G55)},
	MRNUMBER = {3701353},
	MRREVIEWER = {Adrian Langer},
	DOI = {10.1090/surv/221.2},
	URL = {https://doi.org/10.1090/surv/221.2},
}


@book {studyindag1,
	AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
	TITLE = {A study in derived algebraic geometry. {V}ol. {I}.
		{C}orrespondences and duality},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {221},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2017},
	PAGES = {xl+533pp},
	ISBN = {978-1-4704-3569-1},
	MRCLASS = {14F05 (18D05 18G55)},
	MRNUMBER = {3701352},
	MRREVIEWER = {Adrian Langer},
	DOI = {10.1090/surv/221.1},
	URL = {https://doi.org/10.1090/surv/221.1},
}


@book {weibel,
	AUTHOR = {Weibel, Charles A.},
	TITLE = {An introduction to homological algebra},
	SERIES = {Cambridge Studies in Advanced Mathematics},
	VOLUME = {38},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {1994},
	PAGES = {xiv+450},
	ISBN = {0-521-43500-5},
	MRCLASS = {18-01 (16-01 17-01 20-01 55Uxx)},
	MRNUMBER = {1269324},
	MRREVIEWER = {Kenneth A. Brown},
	DOI = {10.1017/CBO9781139644136},
	URL = {https://doi-org.pros.lib.unimi.it/10.1017/CBO9781139644136},
}


@Book{weil,
title      = {Introduction \`a l'\'etude des vari\'et\'es k\"ahl\'eriennes},
publisher  = {Hermann, Paris},
year       = {1958},
author     = {Weil, Andr\'e},
series     = {Publications de l'Institut de Math\'ematique de l'Universit\'e de Nancago, VI. Actualit\'es Sci. Ind. no. 1267},
mrclass    = {57.00},
mrnumber   = {0111056},
mrreviewer = {F. Hirzebruch},
pages      = {175},
}


@book {rosicky,
	AUTHOR = {Ad\'{a}mek, Ji\v{r}\'{\i} and Rosick\'{y}, Ji\v{r}\'{\i}},
	TITLE = {Locally presentable and accessible categories},
	SERIES = {London Mathematical Society Lecture Note Series},
	VOLUME = {189},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {1994},
	PAGES = {xiv+316},
	ISBN = {0-521-42261-2},
	MRCLASS = {18Axx (18-02)},
	MRNUMBER = {1294136},
	MRREVIEWER = {J. R. Isbell},
	DOI = {10.1017/CBO9780511600579},
	URL = {https://doi.org/10.1017/CBO9780511600579},
}


@Book{htt,
AUTHOR = {Lurie, Jacob},
TITLE = {Higher topos theory},
SERIES = {Annals of Mathematics Studies},
VOLUME = {170},
PUBLISHER = {Princeton University Press, Princeton, NJ},
YEAR = {2009},
PAGES = {xviii+925},
ISBN = {978-0-691-14049-0},
MRCLASS = {18-02 (18B25 18E35 18G30 18G55 55U40)},
MRNUMBER = {2522659},
MRREVIEWER = {Mark Hovey},
DOI = {10.1515/9781400830558},
URL = {https://doi.org/10.1515/9781400830558},
}

@article {tstructurektheory,
	AUTHOR = {Antieau, Benjamin and Gepner, David and Heller, Jeremiah},
	TITLE = {{$K$}-theoretic obstructions to bounded {$t$}-structures},
	JOURNAL = {Invent. Math.},
	FJOURNAL = {Inventiones Mathematicae},
	VOLUME = {216},
	YEAR = {2019},
	NUMBER = {1},
	PAGES = {241--300},
	ISSN = {0020-9910},
	MRCLASS = {19D35 (16E45 16P40 18E10 18E30 55P43)},
	MRNUMBER = {3935042},
	MRREVIEWER = {Guillermo Corti\~{n}as},
	DOI = {10.1007/s00222-018-00847-0},
	URL = {https://doi-org.pros2.lib.unimi.it/10.1007/s00222-018-00847-0},
}


@article {gepnerhaugseng,
    AUTHOR = {Gepner, David and Haugseng, Rune},
     TITLE = {Enriched {$\infty$}-categories via non-symmetric
              {$\infty$}-operads},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {279},
      YEAR = {2015},
     PAGES = {575--716},
      ISSN = {0001-8708},
   MRCLASS = {18D20 (18D10 18D50)},
  MRNUMBER = {3345192},
MRREVIEWER = {Christopher L. Rogers},
       DOI = {10.1016/j.aim.2015.02.007},
       URL = {https://doi.org/10.1016/j.aim.2015.02.007},
}


@Misc{ha,
AUTHOR = {Lurie, Jacob},
TITLE = {Higher Algebra},
YEAR = {2017},
PAGES = {1553},
URL = {http://www.math.harvard.edu/~lurie/papers/HA.pdf},
}


@Misc{portasala,
AUTHOR = {Porta, Mauro and Sala, Francesco},
TITLE = {Simpson’s shapes of schemes and stacks},
YEAR = {2020},
URL = {https://people.dm.unipi.it/sala/assets/pdf/porta_sala_shapes.pdf},
}

@misc{carmeli2023characterstransfermapscategorified,
      title={Characters and transfer maps via categorified traces}, 
      author={Shachar Carmeli and Bastiaan Cnossen and Maxime Ramzi and Lior Yanovski},
      year={2023},
      eprint={2210.17364},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2210.17364}, 
}

@misc{benmoshe2024categoricalambidexterity,
      title={Categorical Ambidexterity}, 
      author={Shay Ben-Moshe},
      year={2024},
      eprint={2411.17281},
      archivePrefix={arXiv},
      primaryClass={math.CT},
      url={https://arxiv.org/abs/2411.17281}, 
}


@misc{mazelgee2021universal,
      title={A universal characterization of noncommutative motives and secondary algebraic K-theory}, 
      author={Aaron Mazel-Gee and Reuben Stern},
      year={2021},
      eprint={2104.04021},
      archivePrefix={arXiv},
      primaryClass={math.KT}
}


@article{pare, title={Simply Connected Limits}, volume={42}, DOI={10.4153/CJM-1990-038-6}, number={4}, journal={Canadian Journal of Mathematics}, publisher={Cambridge University Press}, author={Paré, Robert}, year={1990}, pages={731–746}}


@Misc{sag,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Spectral Algebraic Geometry (Under Construction)},
	YEAR = {2018},
	URL = {https://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf},
}


@article{heineenrichedaction,
title = {An equivalence between enriched $\infty$-categories and $\infty$-categories with weak action},
journal = {Advances in Mathematics},
volume = {417},
pages = {108941},
year = {2023},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2023.108941},
url = {https://www.sciencedirect.com/science/article/pii/S0001870823000841},
author = {Hadrian Heine},
}


@misc{schreiber2013differential,
      title={Differential cohomology in a cohesive infinity-topos}, 
      author={Urs Schreiber},
      year={2013},
      eprint={1310.7930},
      archivePrefix={arXiv},
      primaryClass={math-ph}
}


@article {holstein,
    AUTHOR = {Holstein, Julian V. S.},
     TITLE = {Morita cohomology and homotopy locally constant sheaves},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {158},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {27--35},
      ISSN = {0305-0041,1469-8064},
   MRCLASS = {55N30 (18G60)},
  MRNUMBER = {3300313},
MRREVIEWER = {Timothy\ Porter},
       DOI = {10.1017/S0305004114000528},
       URL = {https://doi.org/10.1017/S0305004114000528},
}


@book {sadun,
    AUTHOR = {Sadun, Lorenzo},
     TITLE = {Topology of tiling spaces},
    SERIES = {University Lecture Series},
    VOLUME = {46},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2008},
     PAGES = {x+118},
      ISBN = {978-0-8218-4727-5},
   MRCLASS = {52C22 (37B50 52C23 55N05)},
  MRNUMBER = {2446623},
MRREVIEWER = {Bernd\ Sing},
       DOI = {10.1090/ulect/046},
       URL = {https://doi.org/10.1090/ulect/046},
}


@Misc{dagviii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry VIII: Quasi-Coherent Sheaves and
		Tannaka Duality Theorems},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-VIII.pdf},
}


@Misc{dagvii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry VII: Spectral Schemes},
	YEAR = {2011},
	URL = {https://people.math.harvard.edu/~lurie/papers/DAG-VII.pdf},
}


@Misc{dagx,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry X: Formal Moduli Problems},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-X.pdf},
}

@Misc{dagxiii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry XIII: Rational and $p$-adic Homotopy Theory},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-XIII.pdf},
}



@Misc{ellipticcohomology1,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Elliptic Cohomology I: Spectral Abelian Varieties},
	YEAR = {2018},
	URL = {http://people.math.harvard.edu/~lurie/papers/Elliptic-I.pdf},
}


@Misc{schwedespectra,
	AUTHOR = {Schwede, Stefan},
	TITLE = {Symmetric Spectra},
	YEAR = {2012},
	URL = {http://www.math.uni-bonn.de/people/schwede/SymSpec-v3.pdf},
}


@article {bravdyckerhoff,
AUTHOR = {Brav, Christopher and Dyckerhoff, Tobias},
TITLE = {Relative {C}alabi-{Y}au structures},
JOURNAL = {Compos. Math.},
FJOURNAL = {Compositio Mathematica},
VOLUME = {155},
YEAR = {2019},
NUMBER = {2},
PAGES = {372--412},
ISSN = {0010-437X},
MRCLASS = {18E30 (14F05 32Q25 58B34)},
MRNUMBER = {3911626},
DOI = {10.1112/s0010437x19007024},
URL = {https://doi.org/10.1112/s0010437x19007024},
}


@article {toenvaquie,
AUTHOR = {To\"{e}n, Bertrand and Vaqui\'{e}, Michel},
TITLE = {Moduli of objects in dg-categories},
JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
	S\'{e}rie},
VOLUME = {40},
YEAR = {2007},
NUMBER = {3},
PAGES = {387--444},
ISSN = {0012-9593},
MRCLASS = {18G55 (14D20 18E30)},
MRNUMBER = {2493386},
MRREVIEWER = {Andrey Yu. Lazarev},
DOI = {10.1016/j.ansens.2007.05.001},
URL = {https://doi.org/10.1016/j.ansens.2007.05.001},
}


@article {verdier,
AUTHOR = {Verdier, Jean-Louis},
TITLE = {Des cat\'{e}gories d\'{e}riv\'{e}es des cat\'{e}gories ab\'{e}liennes},
NOTE = {With a preface by Luc Illusie,
	Edited and with a note by Georges Maltsiniotis},
JOURNAL = {Ast\'{e}risque},
FJOURNAL = {Ast\'{e}risque},
NUMBER = {239},
YEAR = {1996},
PAGES = {xii+253 pp. (1997)},
ISSN = {0303-1179},
MRCLASS = {18E30 (18-03 18E35)},
MRNUMBER = {1453167},
MRREVIEWER = {Amnon Neeman},
}




@Article{vialekahn,
author   = {Barbieri-Viale, Luca and Kahn, Bruno},
title    = {On the derived category of 1-motives},
journal  = {Ast\'erisque},
year     = {2016},
number   = {381},
pages    = {xi+254},
issn     = {0303-1179},
fjournal = {Ast\'erisque},
isbn     = {978-2-85629-837-4},
mrclass  = {14F05 (14C30 14F20 18E30)},
mrnumber = {3545132},
}


@Article{vialesrinivas,
author     = {Barbieri-Viale, Luca and Srinivas, Vasudevan},
title      = {Albanese and {P}icard 1-motives},
journal    = {M\'em. Soc. Math. Fr. (N.S.)},
year       = {2001},
number     = {87},
pages      = {vi+104},
issn       = {0249-633X},
fjournal   = {M\'emoires de la Soci\'et\'e Math\'ematique de France. Nouvelle S\'erie},
mrclass    = {14C30 (14F42 14K30)},
mrnumber   = {1891270},
mrreviewer = {Tam\~A!`s Szamuely},
}


@misc{GPS,
    title={Mirror symmetry: from categories to curve counts},
    author={Sheel Ganatra and Timothy Perutz and Nick Sheridan},
    year={2015},
    eprint={1510.03839},
    archivePrefix={arXiv},
    primaryClass={math.SG}
}


@Article{HMS,
author={Haugseng, Rune, and Melani, Valerio and Safronov, Pavel},
title={Shifted coisotropic correspondences},
year={2019},
url={	arXiv:1904.11312},
}


@Article{barbierisaito,
author     = {Barbieri-Viale, L. and Rosenschon, A. and Saito, M.},
title      = {Deligne's conjecture on 1-motives},
journal    = {Ann. of Math. (2)},
year       = {2003},
volume     = {158},
number     = {2},
pages      = {593--633},
issn       = {0003-486X},
doi        = {10.4007/annals.2003.158.593},
fjournal   = {Annals of Mathematics. Second Series},
mrclass    = {14C30 (14D07)},
mrnumber   = {2018930},
mrreviewer = {H\~A\copyright{}l\~A\"{\ }ne Esnault},
url        = {http://dx.doi.org/10.4007/annals.2003.158.593},
}


@Book{berthelot,
title      = {Th\'eorie de {D}ieudonn\'e cristalline. {II}},
publisher  = {Springer-Verlag, Berlin},
year       = {1982},
author     = {Berthelot, Pierre and Breen, Lawrence and Messing, William},
volume     = {930},
series     = {Lecture Notes in Mathematics},
isbn       = {3-540-11556-0},
doi        = {10.1007/BFb0093025},
mrclass    = {14L05 (14F30)},
mrnumber   = {667344},
mrreviewer = {Lucile B\~A\copyright{}gueri},
pages      = {x+261},
url        = {http://dx.doi.org/10.1007/BFb0093025},
}


@Book{neronmodels,
title      = {N\'eron models},
publisher  = {Springer-Verlag, Berlin},
year       = {1990},
author     = {Bosch, Siegfried and L\"utkebohmert, Werner and Raynaud, Michel},
volume     = {21},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results in Mathematics and Related Areas (3)]},
isbn       = {3-540-50587-3},
doi        = {10.1007/978-3-642-51438-8},
mrclass    = {14K15 (11G10 14L15)},
mrnumber   = {1045822},
mrreviewer = {James Milne},
pages      = {x+325},
url        = {http://dx.doi.org/10.1007/978-3-642-51438-8},
}


@Misc{mixedmotives,
author       = {Cisinski, Denis-Charles and Déglise, Frédéric},
title        = {Triangulated categories of mixed motives},
howpublished = {https://arxiv.org/pdf/0912.2110.pdf},
month        = {Dec},
year         = {2012},
publisher    = {arXiv:0912.2110v3},
}


@Article{delignelefschetz,
author     = {Deligne, P.},
title      = {Th\'eor\`eme de {L}efschetz et crit\`eres de d\'eg\'en\'erescence de suites spectrales},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1968},
number     = {35},
pages      = {259--278},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14.52},
mrnumber   = {0244265},
mrreviewer = {D. I. Lieberman},
url        = {http://www.numdam.org/item?id=PMIHES_1968__35__259_0},
}


@Article{hodgetheory2,
author     = {Deligne, Pierre},
title      = {Th\'eorie de {H}odge. {II}},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1971},
number     = {40},
pages      = {5--57},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14C30 (14F15)},
mrnumber   = {0498551},
mrreviewer = {J. H. M. Steenbrink},
url        = {http://www.numdam.org/item?id=PMIHES_1971__40__5_0},
}


@Article{hodgetheory3,
author     = {Deligne, Pierre},
title      = {Th\'eorie de {H}odge. {III}},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1974},
number     = {44},
pages      = {5--77},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14C30 (14F15)},
mrnumber   = {0498551},
mrreviewer = {J. H. M. Steenbrink},
url        = {http://www.numdam.org/item?id=PMIHES_1971__40__5_0},
}


@Misc{moonen,
author       = {Moonen, Ben and van der Geer, Gerard and Edixhoven, Bas},
title        = {Abelian Varieties},
howpublished = {http://www.mi.fu-berlin.de/users/elenalavanda/BMoonen.pdf},
note         = {Preliminary version},
}


@incollection {lipmanadjointassociativity,
	AUTHOR = {Lipman, Joseph},
	TITLE = {Adjoint associativity: an invitation to algebra in
		{$\infty$}-categories},
	BOOKTITLE = {Commutative algebra and noncommutative algebraic geometry.
		{V}ol. {II}},
	SERIES = {Math. Sci. Res. Inst. Publ.},
	VOLUME = {68},
	PAGES = {265--291},
	PUBLISHER = {Cambridge Univ. Press, New York},
	YEAR = {2015},
	MRCLASS = {14F05 (13D03 13D09 18D10 18D35 18G55)},
	MRNUMBER = {3496871},
	MRREVIEWER = {\Dbar \cftil{o} Ng\d{o}c Di\cfudot{e}p},
}

@book {MR0241495,
    AUTHOR = {Grothendieck, A.},
     TITLE = {Cat\'{e}gories cofibr\'{e}es additives et complexe cotangent
              relatif},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {No. 79},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1968},
     PAGES = {ii+167},
   MRCLASS = {18.10 (14.00)},
  MRNUMBER = {241495},
MRREVIEWER = {P.\ Abellanas},
}

@book {complexcotangent2,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {II}},
	SERIES = {Lecture Notes in Mathematics, Vol. 283},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1972},
	PAGES = {vii+304},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491681},
	MRREVIEWER = {Larry Breen},
}

@book {MR0146040,
    AUTHOR = {Grothendieck, Alexander},
     TITLE = {Fondements de la g\'{e}om\'{e}trie alg\'{e}brique. [{E}xtraits
              du {S}\'{e}minaire {B}ourbaki, 1957--1962.]},
 PUBLISHER = {Secr\'{e}tariat math\'{e}matique, Paris},
      YEAR = {1962},
     PAGES = {ii+205},
   MRCLASS = {14.00},
  MRNUMBER = {146040},
}

@article {MR0217093,
    AUTHOR = {Schlessinger, Michael},
     TITLE = {Functors of {A}rtin rings},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {130},
      YEAR = {1968},
     PAGES = {208--222},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {14.55},
  MRNUMBER = {217093},
MRREVIEWER = {M.\ Miyanishi},
       DOI = {10.2307/1994967},
       URL = {https://doi.org/10.2307/1994967},
}

@book {MR0815922,
    AUTHOR = {Kodaira, Kunihiko},
     TITLE = {Complex manifolds and deformation of complex structures},
    SERIES = {Grundlehren der mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {283},
      NOTE = {Translated from the Japanese by Kazuo Akao,
              With an appendix by Daisuke Fujiwara},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1986},
     PAGES = {x+465},
      ISBN = {0-387-96188-7},
   MRCLASS = {32G05 (32-02)},
  MRNUMBER = {815922},
MRREVIEWER = {James\ A.\ Carlson},
       DOI = {10.1007/978-1-4613-8590-5},
       URL = {https://doi.org/10.1007/978-1-4613-8590-5},
}

@article {MR0195995,
    AUTHOR = {Nijenhuis, Albert and Richardson, Jr., R. W.},
     TITLE = {Cohomology and deformations in graded {L}ie algebras},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {72},
      YEAR = {1966},
     PAGES = {1--29},
      ISSN = {0002-9904},
   MRCLASS = {17.30 (16.90)},
  MRNUMBER = {195995},
MRREVIEWER = {G.\ Leger},
       DOI = {10.1090/S0002-9904-1966-11401-5},
       URL = {https://doi.org/10.1090/S0002-9904-1966-11401-5},
}

@article {MR0161898,
    AUTHOR = {Gerstenhaber, Murray},
     TITLE = {The cohomology structure of an associative ring},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {78},
      YEAR = {1963},
     PAGES = {267--288},
      ISSN = {0003-486X},
   MRCLASS = {16.90 (18.00)},
  MRNUMBER = {161898},
MRREVIEWER = {M.\ Auslander},
       DOI = {10.2307/1970343},
       URL = {https://doi.org/10.2307/1970343},
}

@article {MR0171807,
    AUTHOR = {Gerstenhaber, Murray},
     TITLE = {On the deformation of rings and algebras},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {79},
      YEAR = {1964},
     PAGES = {59--103},
      ISSN = {0003-486X},
   MRCLASS = {16.90 (13.93)},
  MRNUMBER = {171807},
MRREVIEWER = {D.\ Zelinsky},
       DOI = {10.2307/1970484},
       URL = {https://doi.org/10.2307/1970484},
}

@article {MR0083801,
    AUTHOR = {Fr\"{o}licher, Alfred and Nijenhuis, Albert},
     TITLE = {A theorem on stability of complex structures},
   JOURNAL = {Proc. Nat. Acad. Sci. U.S.A.},
  FJOURNAL = {Proceedings of the National Academy of Sciences of the United
              States of America},
    VOLUME = {43},
      YEAR = {1957},
     PAGES = {239--241},
      ISSN = {0027-8424},
   MRCLASS = {53.3X},
  MRNUMBER = {83801},
MRREVIEWER = {M.\ F.\ Atiyah},
       DOI = {10.1073/pnas.43.2.239},
       URL = {https://doi.org/10.1073/pnas.43.2.239},
}

@Article{zbMATH02694718,
 Author = {Noether, M.},
 Title = {Anzahl der {Moduln} einer {Klasse} algebraischer {Fl{\"a}chen}.},
 FJournal = {Sitzungsberichte der K{\"o}niglich Preussischen Akademie der Wissenschaften},
 Journal = {Berl. Ber.},
 Volume = {1888},
 Pages = {123--128},
 Year = {1888},
 Language = {German},
 zbMATH = {2694718},
 JFM = {20.0794.04}
}

@article {MR1579035,
    AUTHOR = {Riemann, B.},
     TITLE = {Theorie der {A}bel'schen {F}unctionen},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {54},
      YEAR = {1857},
     PAGES = {115--155},
      ISSN = {0075-4102,1435-5345},
   MRCLASS = {99-04},
  MRNUMBER = {1579035},
       DOI = {10.1515/crll.1857.54.115},
       URL = {https://doi.org/10.1515/crll.1857.54.115},
}

@article {DDT,
	AUTHOR = {Drinfeld, V.},
	TITLE = {A letter from {K}harkov to {M}oscow},
	NOTE = {Translated from the Russian by Keith Conrad},
	JOURNAL = {EMS Surv. Math. Sci.},
	FJOURNAL = {EMS Surveys in Mathematical Sciences},
	VOLUME = {1},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {241--248},
	ISSN = {2308-2151},
	MRCLASS = {18G55 (14D15 17B55)},
	MRNUMBER = {3285856},
	DOI = {10.4171/EMSS/5},
	URL = {https://doi.org/10.4171/EMSS/5},
}

@article {KodairaSpencer,
	AUTHOR = {Kodaira, K. and Spencer, D. C.},
	TITLE = {On deformations of complex analytic structures. {I}, {II}},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {67},
	YEAR = {1958},
	PAGES = {328--466},
	ISSN = {0003-486X},
	MRCLASS = {57.00},
	MRNUMBER = {112154},
	MRREVIEWER = {M. F. Atiyah},
	DOI = {10.2307/1970009},
	URL = {https://doi.org/10.2307/1970009},
}

@article {toen_azumaya,
    AUTHOR = {To\"en, Bertrand},
     TITLE = {Derived {A}zumaya algebras and generators for twisted derived
              categories},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {189},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {581--652},
      ISSN = {0020-9910,1432-1297},
   MRCLASS = {18E30 (14F05 14F20 16E35 18D10 18G55)},
  MRNUMBER = {2957304},
MRREVIEWER = {Julia\ Bergner},
       DOI = {10.1007/s00222-011-0372-1},
       URL = {https://doi.org/10.1007/s00222-011-0372-1},
}

@article {antieau_gepner_brauer_groups,
    AUTHOR = {Antieau, Benjamin and Gepner, David},
     TITLE = {Brauer groups and \'etale cohomology in derived algebraic
              geometry},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {18},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {1149--1244},
      ISSN = {1465-3060,1364-0380},
   MRCLASS = {14F22 (13D09 14D20 18G55 55P43)},
  MRNUMBER = {3190610},
MRREVIEWER = {Timothy\ J.\ Ford},
       DOI = {10.2140/gt.2014.18.1149},
       URL = {https://doi.org/10.2140/gt.2014.18.1149},
}


@article {hinich,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {Homological algebra of homotopy algebras},
	JOURNAL = {Comm. Algebra},
	FJOURNAL = {Communications in Algebra},
	VOLUME = {25},
	YEAR = {1997},
	NUMBER = {10},
	PAGES = {3291--3323},
	ISSN = {0092-7872},
	MRCLASS = {18G99 (16E99 18G05 55U35)},
	MRNUMBER = {1465117},
	MRREVIEWER = {Kathryn P. Hess},
	DOI = {10.1080/00927879708826055},
	URL = {https://doi.org/10.1080/00927879708826055},
}


@article {hinichcoalgebras,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {D{G} coalgebras as formal stacks},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {162},
	YEAR = {2001},
	NUMBER = {2-3},
	PAGES = {209--250},
	ISSN = {0022-4049},
	MRCLASS = {14B12 (16W30 18G55 55P62)},
	MRNUMBER = {1843805},
	MRREVIEWER = {Paul G. Goerss},
	DOI = {10.1016/S0022-4049(00)00121-3},
	URL = {https://doi.org/10.1016/S0022-4049(00)00121-3},
}


@article {pridham,
	AUTHOR = {Pridham, J. P.},
	TITLE = {Unifying derived deformation theories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {224},
	YEAR = {2010},
	NUMBER = {3},
	PAGES = {772--826},
	ISSN = {0001-8708},
	MRCLASS = {14B12 (16E35)},
	MRNUMBER = {2628795},
	MRREVIEWER = {Eivind Eriksen},
	DOI = {10.1016/j.aim.2009.12.009},
	URL = {https://doi.org/10.1016/j.aim.2009.12.009},
}


@article {dagsurvey,
	AUTHOR = {To\"{e}n, Bertrand},
	TITLE = {Derived algebraic geometry},
	JOURNAL = {EMS Surv. Math. Sci.},
	FJOURNAL = {EMS Surveys in Mathematical Sciences},
	VOLUME = {1},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {153--240},
	ISSN = {2308-2151},
	MRCLASS = {14A20 (14D15 18G55)},
	MRNUMBER = {3285853},
	MRREVIEWER = {Julia Bergner},
	DOI = {10.4171/EMSS/4},
	URL = {https://doi.org/10.4171/EMSS/4},
}


@book {complexcotangent1,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {I}},
	SERIES = {Lecture Notes in Mathematics, Vol. 239},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1971},
	PAGES = {xv+355},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491680},
	MRREVIEWER = {Larry Breen},
}


@misc{gammage2023perverse,
      title={Perverse schobers and 3d mirror symmetry}, 
      author={Benjamin Gammage and Justin Hilburn and Aaron Mazel-Gee},
      year={2023},
      eprint={2202.06833},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}


@Book{fgaexplained,
title      = {Fundamental algebraic geometry},
publisher  = {American Mathematical Society, Providence, RI},
year       = {2005},
author     = {Fantechi, Barbara and G\"ottsche, Lothar and Illusie, Luc and Kleiman, Steven L. and Nitsure, Nitin and Vistoli, Angelo},
volume     = {123},
series     = {Mathematical Surveys and Monographs},
isbn       = {0-8218-3541-6},
note       = {Grothendieck's FGA explained},
mrclass    = {14-06 (14A15 14D15 14F20)},
mrnumber   = {2222646},
mrreviewer = {Liam O'Carroll},
pages      = {x+339},
}


@misc{CG,
	title={Formal moduli problems and formal derived stacks}, 
	author={Damien Calaque and Julien Grivaux},
	year={2019},
	eprint={1802.09556},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@Book{fga,
title      = {Fondements de la g\'eom\'etrie alg\'ebrique. [{E}xtraits du {S}\'eminaire {B}ourbaki, 1957--1962.]},
publisher  = {Secr\'etariat math\'ematique, Paris},
year       = {1962},
author     = {Grothendieck, Alexander},
mrclass    = {14.00},
mrnumber   = {0146040},
mrreviewer = {E. L. Griffin, Jr.},
pages      = {ii+205},
}


@InCollection{descente,
author    = {Grothendieck, Alexander},
title     = {Technique de descente et th\'eor\`emes d'existence en g\'eometrie alg\'ebrique. {I}. {G}\'en\'eralit\'es. {D}escente par morphismes fid\`element plats},
booktitle = {S\'eminaire {B}ourbaki, {V}ol.\ 5},
publisher = {Soc. Math. France, Paris},
year      = {1995},
pages     = {Exp.\ No.\ 190, 299--327},
mrclass   = {14A15},
mrnumber  = {1603475},
}


@Book{hartshorne,
title      = {Algebraic geometry},
publisher  = {Springer-Verlag, New York-Heidelberg},
year       = {1977},
author     = {Hartshorne, Robin},
isbn       = {0-387-90244-9},
note       = {Graduate Texts in Mathematics, No. 52},
mrclass    = {14-01},
mrnumber   = {0463157},
mrreviewer = {Robert Speiser},
pages      = {xvi+496},
}


@Book{hodge,
title     = {The theory and applications of harmonic integrals},
publisher = {Cambridge University Press, Cambridge},
year      = {1989},
author    = {Hodge, W. V. D.},
series    = {Cambridge Mathematical Library},
isbn      = {0-521-35881-7},
note      = {Reprint of the 1941 original, With a foreword by Michael Atiyah},
mrclass   = {58A14 (01A60 01A75 32G20 53-02)},
mrnumber  = {1015714},
pages     = {xiv+284},
}


@Article{hironaka,
author     = {Hironaka, Heisuke},
title      = {Resolution of singularities of an algebraic variety over a field of characteristic zero. {I}, {II}},
journal    = {Ann. of Math. (2) {\bf 79} (1964), 109--203; ibid. (2)},
year       = {1964},
volume     = {79},
pages      = {205--326},
issn       = {0003-486X},
fjournal   = {Annals of Mathematics. Second Series},
mrclass    = {14.18},
mrnumber   = {0199184},
mrreviewer = {J. Giraud},
}


@Book{liu,
title      = {Algebraic geometry and arithmetic curves},
publisher  = {Oxford University Press, Oxford},
year       = {2002},
author     = {Liu, Qing},
volume     = {6},
series     = {Oxford Graduate Texts in Mathematics},
isbn       = {0-19-850284-2},
note       = {Translated from the French by Reinie Ern\'e, Oxford Science Publications},
mrclass    = {14-01 (11G30 14A05 14A15 14Gxx 14Hxx)},
mrnumber   = {1917232},
mrreviewer = {C\~A-cero Carvalho},
pages      = {xvi+576},
}


@Book{mazurmessing,
title      = {Universal extensions and one dimensional crystalline cohomology},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1974},
author     = {Mazur, B. and Messing, William},
series     = {Lecture Notes in Mathematics, Vol. 370},
mrclass    = {14K05 (14F30 14G05 14L05)},
mrnumber   = {0374150},
mrreviewer = {S. Bloch},
pages      = {vii+134},
}


@Book{mumford,
title      = {Geometric invariant theory},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1965},
author     = {Mumford, David},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete, Neue Folge, Band 34},
mrclass    = {14.55},
mrnumber   = {0214602},
mrreviewer = {F. Oort},
pages      = {vi+145},
}


@Article{murre,
author     = {Murre, J. P.},
title      = {On contravariant functors from the category of pre-schemes over a field into the category of abelian groups (with an application to the {P}icard functor)},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1964},
number     = {23},
pages      = {5--43},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14.55},
mrnumber   = {0206011},
mrreviewer = {J. R. Isbell},
url        = {http://www.numdam.org/item?id=PMIHES_1964__23__5_0},
}


@Article{Oort,
author     = {Oort, F.},
title      = {Algebraic group schemes in characteristic zero are reduced},
journal    = {Invent. Math.},
year       = {1966},
volume     = {2},
pages      = {79--80},
issn       = {0020-9910},
doi        = {10.1007/BF01403391},
fjournal   = {Inventiones Mathematicae},
mrclass    = {14.50},
mrnumber   = {0206005},
mrreviewer = {S. S. Shatz},
url        = {http://dx.doi.org/10.1007/BF01403391},
}


@Book{oort2,
title         = {Commutative group schemes},
publisher     = {Springer-Verlag, Berlin-New York},
year          = {1966},
author        = {Oort, F.},
volume        = {15},
series        = {Lecture Notes in Mathematics},
__markedentry = {[Emanuele:1]},
mrclass       = {14.50 (18.00)},
mrnumber      = {0213365},
mrreviewer    = {S. S. Shatz},
pages         = {vi+133 pp. (not consecutively paged)},
}


@Book{steenbrink,
title      = {Mixed {H}odge structures},
publisher  = {Springer-Verlag, Berlin},
year       = {2008},
author     = {Peters, Chris A. M. and Steenbrink, Joseph H. M.},
volume     = {52},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in Mathematics [Results in Mathematics and Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
isbn       = {978-3-540-77015-2},
mrclass    = {14C30 (14D07 32G20 32J25 32S35)},
mrnumber   = {2393625},
mrreviewer = {Matt Kerr},
pages      = {xiv+470},
}


@Book{raynaud,
title      = {Faisceaux amples sur les sch\'emas en groupes et les espaces homog\`enes},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1970},
author     = {Raynaud, Michel},
series     = {Lecture Notes in Mathematics, Vol. 119},
mrclass    = {14.55},
mrnumber   = {0260758},
mrreviewer = {D. Gieseker},
pages      = {ii+218},
}


@Article{gaga,
author     = {Serre, Jean-Pierre},
title      = {G\'eom\'etrie alg\'ebrique et g\'eom\'etrie analytique},
journal    = {Ann. Inst. Fourier, Grenoble},
year       = {1955--1956},
volume     = {6},
pages      = {1--42},
issn       = {0373-0956},
fjournal   = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
mrclass    = {53.3X},
mrnumber   = {0082175},
mrreviewer = {H. Cartan},
url        = {http://aif.cedram.org/item?id=AIF_1955__6__1_0},
}


@Book{motives,
title      = {Cycles, transfers, and motivic homology theories},
publisher  = {Princeton University Press, Princeton, NJ},
year       = {2000},
author     = {Voevodsky, Vladimir and Suslin, Andrei and Friedlander, Eric M.},
volume     = {143},
series     = {Annals of Mathematics Studies},
isbn       = {0-691-04814-2; 0-691-04815-0},
mrclass    = {14F42 (14C25 19E15)},
mrnumber   = {1764197},
mrreviewer = {Spencer J. Bloch},
pages      = {vi+254},
}


@Book{sga3,
title     = {S\'eminaire de G\'eom\'etrie Alg\'ebrique du Bois-Marie},
publisher = {Springer-Verlag},
year      = {1970-1973},
author    = {Grothendieck, Alexander and Raynaud, Mich\`ele and Demazure, Michel and Artin, Michael and Verdier, Jean-Louis and Deligne, Pierre and Berthelot, Pierre and Illusie, Luc and Katz, Nicholas},
address   = {Berlin},
note      = {Lecture Notes in Mathematics, Vols. 151, 152, 153, 224, 225, 269, 270, 288, 305, 340, 569, and 589},
}


@Book{ega,
title     = {\'{E}l\'ements de g\'eom\'etrie alg\'ebrique.},
publisher = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year      = {1960-1967},
author    = {Grothendieck, Alexander and Dieudonn\'e, Jean-Alexandre-Eug\`ene},
number    = {4, 8, 11, 17, 20, 24, 28, and 32},
note      = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
fjournal  = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
issn      = {0073-8301},
mrclass   = {14.55},
}


@Misc{milne2,
author       = {Milne, James S.},
title        = {Algebraic Groups},
howpublished = {http://www.jmilne.org/math/CourseNotes/iAG200.pdf},
month        = {Dec},
year         = {2015},
}


@Misc{pink,
author       = {Pink, Richard},
title        = {Finite group schemes},
howpublished = {https://people.math.ethz.ch/~pink/ftp/FGS/CompleteNotes.pdf},
year         = {2004/2005},
note         = {Lecture notes.},
}


@Article{andre,
author  = {Yves Andr\`e},
title   = {Une introduction aux motifs (motifs purs, motifs mixtes, p\`eriodes)},
journal = {Panoramas et Synth\'eses [Panoramas and Syntheses], vol. 17},
year    = {2004},
}


@Article{tabuada,
author  = {Gonçalo Tabuada},
title   = {Noncommutative Motives},
journal = {American Mathematical Society University Lecture Series},
year    = {2010},
volume  = {63},
}


@Misc{voevconjecture,
author       = {Marcello Bernardara, and Matilde Marcolli, and Gonçalo Tabuada},
title        = {Some remarks concerning Voevodsky’s nilpotence conjecture},
howpublished = {https://arxiv.org/pdf/0912.2110.pdf},
journal      = {arXiv:1403.0876(v3).},
}


@Article{kahnsebastian,
author  = {Bruno Kahn and Ronnie Sebastian},
title   = {Smash-nilpotent cycles on abelian 3-folds},
journal = {Math. Res. Lett. 16},
year    = {2009},
volume  = {6},
pages   = {1007–1010},
}


@Article{matsusaka,
author  = {Teruhisa Matsusaka},
title   = {The criteria for algebraic equivalence and the torsion group},
journal = {Amer. J. Math. 79},
year    = {1957},
pages   = {53-66},
}


@Article{voevodskynilpotence,
author  = {Vladimir Voevodsky},
title   = {A nilpotence theorem for cycles algebraically equivalent to zero},
journal = {Internat. Math. Res. Notices},
year    = {1995},
volume  = {4},
pages   = {187-198},
}


@article {joyce,
AUTHOR = {Brav, Christopher and Bussi, Vittoria and Joyce, Dominic},
TITLE = {A {D}arboux theorem for derived schemes with shifted
	symplectic structure},
JOURNAL = {J. Amer. Math. Soc.},
FJOURNAL = {Journal of the American Mathematical Society},
VOLUME = {32},
YEAR = {2019},
NUMBER = {2},
PAGES = {399--443},
ISSN = {0894-0347},
MRCLASS = {14A20 (14D23 14F05 14N35)},
MRNUMBER = {3904157},
MRREVIEWER = {Hsian-Hua Tseng},
DOI = {10.1090/jams/910},
URL = {https://doi.org/10.1090/jams/910},
}


@book{chriss2009representation,
  title={Representation Theory and Complex Geometry},
  author={Chriss, N. and Ginzburg, V.},
  isbn={9780817649388},
  lccn={94027574},
  series={Modern Birkh{\"a}user Classics},
  url={https://books.google.it/books?id=OZlCAAAAQBAJ},
  year={2009},
  publisher={Birkh{\"a}user Boston}
}




@Misc{rozenblyum2018talk,
AUTHOR = {Rozenblyum, Nick},
TITLE = {Topological Chiral Categories},
YEAR = {2018},
NOTE = {Winter school on local geometric Langlands theory},
URL = {https://lysenko.perso.math.cnrs.fr/Notes_talks_winter2018/T-5(Nick).pdf},
}


@misc{hedenlund2023twisted,
      title={Twisted Spectra Revisited}, 
      author={Alice Hedenlund and Tasos Moulinos},
      year={2023},
      eprint={2312.07403},
      archivePrefix={arXiv},
      primaryClass={math.AT}
}


@incollection {hopfgalois,
	AUTHOR = {Hess, Kathryn},
	TITLE = {Homotopic {H}opf-{G}alois extensions: foundations and
		examples},
	BOOKTITLE = {New topological contexts for {G}alois theory and algebraic
		geometry ({BIRS} 2008)},
	SERIES = {Geom. Topol. Monogr.},
	VOLUME = {16},
	PAGES = {79--132},
	PUBLISHER = {Geom. Topol. Publ., Coventry},
	YEAR = {2009},
	MRCLASS = {55P42 (16T05 18D10 55U35 57T30)},
	MRNUMBER = {2544387},
	MRREVIEWER = {John Hunton},
	DOI = {10.2140/gtm.2009.16.79},
	URL = {https://doi.org/10.2140/gtm.2009.16.79},
}


@article {hinichyoneda,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {Yoneda lemma for enriched {$\infty$}-categories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {367},
	YEAR = {2020},
	PAGES = {107129, 119},
	ISSN = {0001-8708,1090-2082},
	MRCLASS = {18D20 (18M05)},
	MRNUMBER = {4080581},
	MRREVIEWER = {Luciano\ Stramaccia},
	DOI = {10.1016/j.aim.2020.107129},
	URL = {https://doi.org/10.1016/j.aim.2020.107129},
}


@article {dgcoalgebrasformalstacks,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {D{G} coalgebras as formal stacks},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {162},
	YEAR = {2001},
	NUMBER = {2-3},
	PAGES = {209--250},
	ISSN = {0022-4049},
	MRCLASS = {14B12 (16W30 18G55 55P62)},
	MRNUMBER = {1843805},
	MRREVIEWER = {Paul G. Goerss},
	DOI = {10.1016/S0022-4049(00)00121-3},
	URL = {https://doi.org/10.1016/S0022-4049(00)00121-3},
}


@book {weilhodge,
AUTHOR = {Weil, Andr\'{e}},
TITLE = {Introduction \`a l'\'{e}tude des vari\'{e}t\'{e}s k\"{a}hl\'{e}riennes},
SERIES = {Publications de l'Institut de Math\'{e}matique de l'Universit\'{e} de
	Nancago, VI. Actualit\'{e}s Sci. Ind. no. 1267},
PUBLISHER = {Hermann, Paris},
YEAR = {1958},
PAGES = {175},
MRCLASS = {57.00},
MRNUMBER = {0111056},
MRREVIEWER = {F. Hirzebruch},
}


@article {stanculescu,
	AUTHOR = {Stanculescu, Alexandru E.},
	TITLE = {A {Q}uillen model category structure on some categories of
		comonoids},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {214},
	YEAR = {2010},
	NUMBER = {5},
	PAGES = {629--633},
	ISSN = {0022-4049},
	MRCLASS = {55U35},
	MRNUMBER = {2577669},
	DOI = {10.1016/j.jpaa.2009.07.002},
	URL = {https://doi.org/10.1016/j.jpaa.2009.07.002},
}


@book {hirschhorn,
	AUTHOR = {Hirschhorn, Philip S.},
	TITLE = {Model categories and their localizations},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {99},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2003},
	PAGES = {xvi+457},
	ISBN = {0-8218-3279-4},
	MRCLASS = {18G55 (55P60 55U35)},
	MRNUMBER = {1944041},
	MRREVIEWER = {David A. Blanc},
	DOI = {10.1090/surv/099},
	URL = {https://doi.org/10.1090/surv/099},
}


@Article{voisin,
author  = {Claire Voisin},
title   = {Remarks on zero-cycles of self-products of varieties, Moduli of vector bundles},
journal = {Lecture Notes in Pure and Appl. Math.},
year    = {1994},
volume  = {179},
pages   = {265-285},
}


@Article{poonen,
author  = {Bjorn Poonen},
title   = {The Grothendieck ring of varieties is not a domain},
journal = {Math. Res. Lett. 9},
year    = {2002},
volume  = {4},
pages   = {493-497},
}


@Article{bll,
author  = {Alexey I. Bondal, and Michael Larsen, and Valery A. Lunts},
title   = {Grothendieck ring of pretriangulated categories},
journal = {Int. Math. Res. Not.},
year    = {2004},
volume  = {29},
pages   = {1461–1495},
}


@Misc{kuznetsov,
author       = {Alexander Kuznetsov},
title        = {Derived Categories of Quadric Fibrations and Intersections of Quadrics},
howpublished = {arXiv:math/0510670},
month        = oct,
year         = {2005},
}


@book {mcduff-salamon,
    AUTHOR = {McDuff, Dusa and Salamon, Dietmar},
     TITLE = {Introduction to symplectic topology},
    SERIES = {Oxford Mathematical Monographs},
   EDITION = {Second},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {1998},
     PAGES = {x+486},
      ISBN = {0-19-850451-9},
   MRCLASS = {53D35 (53D40 57R17 57R57 57R58)},
  MRNUMBER = {1698616},
MRREVIEWER = {Hansj\"org\ Geiges},
}


@article {savelyev,
    AUTHOR = {Savelyev, Yasha},
     TITLE = {Global {F}ukaya category {I}},
   JOURNAL = {Int. Math. Res. Not. IMRN},
  FJOURNAL = {International Mathematics Research Notices. IMRN},
      YEAR = {2023},
    NUMBER = {21},
     PAGES = {18302--18386},
      ISSN = {1073-7928,1687-0247},
   MRCLASS = {14F08 (18G70 18N20 53D05 53D37)},
  MRNUMBER = {4665626},
       DOI = {10.1093/imrn/rnad013},
       URL = {https://doi.org/10.1093/imrn/rnad013},
}


@article {oh-tanaka,
    AUTHOR = {Oh, Yong-Geun and Tanaka, Hiro Lee},
     TITLE = {Smooth constructions of homotopy-coherent actions},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {22},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {1177--1216},
      ISSN = {1472-2747,1472-2739},
   MRCLASS = {58B05 (53D37 58D05)},
  MRNUMBER = {4474782},
       DOI = {10.2140/agt.2022.22.1177},
       URL = {https://doi.org/10.2140/agt.2022.22.1177},
}

@article {serre_homotopy_groups,
    AUTHOR = {Serre, Jean-Pierre},
     TITLE = {Groupes d'homotopie et classes de groupes ab\'eliens},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {58},
      YEAR = {1953},
     PAGES = {258--294},
      ISSN = {0003-486X},
   MRCLASS = {56.0X},
  MRNUMBER = {59548},
MRREVIEWER = {W.\ S.\ Massey},
       DOI = {10.2307/1969789},
       URL = {https://doi.org/10.2307/1969789},
}

@book {May_Ponto,
    AUTHOR = {May, J. P. and Ponto, K.},
     TITLE = {More concise algebraic topology},
    SERIES = {Chicago Lectures in Mathematics},
      NOTE = {Localization, completion, and model categories},
 PUBLISHER = {University of Chicago Press, Chicago, IL},
      YEAR = {2012},
     PAGES = {xxviii+514},
      ISBN = {978-0-226-51178-8; 0-226-51178-2},
   MRCLASS = {55-02 (16T05 18G55 55P60)},
  MRNUMBER = {2884233},
MRREVIEWER = {Ismar\ Voli\'c},
}

@book {FHTrational,
    AUTHOR = {F\'elix, Yves and Halperin, Stephen and Thomas, Jean-Claude},
     TITLE = {Rational homotopy theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {205},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {2001},
     PAGES = {xxxiv+535},
      ISBN = {0-387-95068-0},
   MRCLASS = {55P62 (18Gxx 55U35)},
  MRNUMBER = {1802847},
MRREVIEWER = {John\ F.\ Oprea},
       DOI = {10.1007/978-1-4613-0105-9},
       URL = {https://doi.org/10.1007/978-1-4613-0105-9},
}

@article {Vigue-Poirrier_Sullivan,
    AUTHOR = {Vigu\'e-Poirrier, Micheline and Sullivan, Dennis},
     TITLE = {The homology theory of the closed geodesic problem},
   JOURNAL = {J. Differential Geometry},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {11},
      YEAR = {1976},
    NUMBER = {4},
     PAGES = {633--644},
      ISSN = {0022-040X,1945-743X},
   MRCLASS = {58E10},
  MRNUMBER = {455028},
MRREVIEWER = {Peter\ Klein},
       URL = {http://projecteuclid.org/euclid.jdg/1214433729},
}

@incollection {Hess_Rational,
    AUTHOR = {Hess, Kathryn},
     TITLE = {Rational homotopy theory: a brief introduction},
 BOOKTITLE = {Interactions between homotopy theory and algebra},
    SERIES = {Contemp. Math.},
    VOLUME = {436},
     PAGES = {175--202},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2007},
      ISBN = {978-0-8218-3814-3},
   MRCLASS = {55P62 (55M30)},
  MRNUMBER = {2355774},
MRREVIEWER = {Yves\ F\'elix},
       DOI = {10.1090/conm/436/08409},
       URL = {https://doi.org/10.1090/conm/436/08409},
}

@article {ayala-francis,
    AUTHOR = {Ayala, David and Francis, John},
     TITLE = {Factorization homology of topological manifolds},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {8},
      YEAR = {2015},
    NUMBER = {4},
     PAGES = {1045--1084},
      ISSN = {1753-8416,1753-8424},
   MRCLASS = {55U40 (57N35 57R19 57R56)},
  MRNUMBER = {3431668},
MRREVIEWER = {Jason\ Stuart\ Hanson},
       DOI = {10.1112/jtopol/jtv028},
       URL = {https://doi.org/10.1112/jtopol/jtv028},
}


@Comment{jabref-meta: databaseType:bibtex;}

